Virtual Constraints and Hybrid Zero Dynamics for Realizing Underactuated Bipedal Locomotion

Underactuation is ubiquitous in human locomotion and should be ubiquitous in bipedal robotic locomotion as well. This chapter presents a coherent theory for the design of feedback controllers that achieve stable walking gaits in underactuated bipedal robots. Two fundamental tools are introduced, virtual constraints and hybrid zero dynamics. Virtual constraints are relations on the state variables of a mechanical model that are imposed through a time-invariant feedback controller. One of their roles is to synchronize the robot's joints to an internal gait phasing variable. A second role is to induce a low dimensional system, the zero dynamics, that captures the underactuated aspects of a robot's model, without any approximations. To enhance intuition, the relation between physical constraints and virtual constraints is first established. From here, the hybrid zero dynamics of an underactuated bipedal model is developed, and its fundamental role in the design of asymptotically stable walking motions is established. The chapter includes numerous references to robots on which the highlighted techniques have been implemented.

==> sections/3b-PhysicalConstraints.tex <==

This section reviews how holonomic constraints in a Lagrangian model yield a reduced-order (exact) model. Consider a Lagrangian system
\begin{equation}
\label{eqn:grizzle:LagrangeNoControl}
D(q) \ddot{q} + C(q,\dot{q})\dot{q} + G(q) = 0,
\end{equation}
with configuration variables $q\in Q$, an open subset of $\mathbb{R}^N$. A \textit{regular holonomic constraint} is a continuously-differentiable  function $h:Q \to \mathbb{R}^k$
such that 
\begin{equation}
\label{eqn:grizzle:ConstraintManifold}
\tilde{Q}=\left\{q \in Q~|~h(q) = 0  \right\}
\end{equation}
is non-empty and for each $q_0\in \tilde{Q}$
\begin{equation}
\label{eqn:grizzle:ConstantRank}
\mathrm{rank}~\frac{\partial h (q_0)}{\partial q}=k.
\end{equation}

The model \eqref{eqn:grizzle:LagrangeNoControl} has a natural restriction to $T\tilde{Q}$ as a mechanical system with $(N-k)$ DOF. To compute it, the principle of virtual work says to augment \eqref{eqn:grizzle:LagrangeNoControl} with a Lagrange multiplier \begin{equation}
\label{eqn:grizzle:LagrangeNoControlWithMultiplier}
D(q) \ddot{q} + C(q,\dot{q})\dot{q} + G(q) = \left(\frac{\partial h(q)}{\partial q}\right)^T \lambda,
\end{equation}
where $\lambda$ is obtained by setting the second derivative of the constraint along solutions of the model to zero, that is,
\begin{align}
0 &= \frac{d^2h}{dt^2} \nonumber \\
\label{eqn:grizzle:SetAccelerationZero}
&= \frac{\partial h(q)}{\partial q} \ddot{q} + \frac{\partial }{\partial q}\left( \frac{\partial h(q)}{\partial q}\dot{q} \right)\dot{q}.
\end{align}
The explicit calculation of $\lambda$ is not necessary here, but can be found in the Appendix.

 
 
 The expression for the reduced-order model can be made more explicit if we assume for simplicity that the holonomic constraint can be expressed as
\begin{equation}
\label{eqn:grizzle:HolonomicConstraintInq1q2}
0=h(q_1,q_2) = q_1 - h_d(q_2),
\end{equation}
 for a choice of configuration variables $q=(q_1,q_2)$, with $q_1 \in \mathbb{R}^k$, $q_2 \in \mathbb{R}^{N-k}$. In this case, the constraint is always regular and the constraint manifold becomes
\begin{equation}
\label{eqn:grizzle:ConstraintManifoldInq1q2}
\tilde{Q}=\left\{(q_1, q_2) \in Q~|~ q_1 = h_d(q_2)  \right\}.
\end{equation}
 
Assuming that the model is partitioned in a manner compatible with the coordinates, that is,
%\begin{equation}
%\label{eqn:grizzle:DInq1q2}
%D(q_1,q_2)=\left[\begin{array}{cc} D_{11}(q_1,q_2) & D_{12}(q_1,q_2) \\   D_{21}(q_1,q_2) & D_{22}(q_1,q_2)\end{array}  \right],
%\end{equation}
\begin{equation}
\label{eqn:grizzle:DInq1q2}
D(q)=\left[\begin{array}{cc} D_{11}(q) & D_{12}(q) \\   D_{21}(q) & D_{22}(q)\end{array}  \right],
\end{equation}
and similarly for $H(q,\dot{q})=C(q,\dot{q})\dot{q} + G(q)$. Then the reduced-order model on $T\tilde{Q}$ can be written as
\begin{equation}
\label{eqn:grizzle:ReducedMechanicalModel}
\tilde{D}(q_2) \ddot{q}_2 + \tilde{H}(q_2, \dot{q}_2)=0,
\end{equation}
where
$$ \tilde{D}(q_2) = \left. \left[ D_{22}(q) + D_{21}(q) \frac{\partial h_d(q_2)}{\partial q_2}  \right] \right|_{q_1 = h_d(q_2)}$$
and
$$ \tilde{H}(q_2, \dot{q}_2) = ??? .$$

The solutions of the reduced-order model \eqref{eqn:grizzle:ReducedMechanicalModel} are (exact) solutions to the full-order model \eqref{eqn:grizzle:LagrangeNoControlWithMultiplier}. Indeed, if $(q_2(t),\dot{q}_2(t))$ is a solution of \eqref{eqn:grizzle:ReducedMechanicalModel}, then 
\begin{align}
q(t) & = \left[\begin{array}{ll} q_1(t) \\ q_2(t) \end{array}  \right]= \left[\begin{array}{cc} h_d(q_2(t)) \\ q_2(t) \end{array}  \right]\\
\dot{q}(t) & = \left[\begin{array}{ll} \dot{q}_1(t) \\ \dot{q}_2(t) \end{array}  \right]= \left[\begin{array}{cc} \frac{\partial h_d(q_2(t))}{\partial q_2} \dot{q}_2(t) \\ \dot{q}_2(t) \end{array}  \right]
\end{align}
is a solution of \eqref{eqn:grizzle:LagrangeNoControlWithMultiplier} with the Lagrange multiplier equal to 
the unique solution of \eqref{eqn:grizzle:SetAccelerationZero}.




==> sections/4-PhysicalConstraintsCC.tex <==

This section reviews how holonomic constraints in a standard Lagrangian model without control inputs induce a reduced-order (exact) model. Consider a Lagrangian system
\begin{equation}
\label{eqn:grizzle:LagrangeNoControl}
D(q) \ddot{q} + C(q,\dot{q})\dot{q} + G(q) = 0,
\end{equation}
with configuration variables $q\in \Q$, an open subset of $\mathbb{R}^N$. A \textit{regular holonomic constraint} is a twice continuously differentiable  function $h:\Q \to \mathbb{R}^k$
such that
\begin{equation}
\label{eqn:grizzle:ConstraintManifold}
\tilde{\Q}=\left\{q \in \Q~|~h(q) = 0  \right\}
\end{equation}
is non-empty and for each $q_0\in \tilde{\Q}$
\begin{equation}
\label{eqn:grizzle:ConstantRank}
\mathrm{rank}~\frac{\partial h (q_0)}{\partial q}=k.
\end{equation}

The model \eqref{eqn:grizzle:LagrangeNoControl} has a natural restriction to $T\tilde{\Q}$ as a mechanical system with $(N-k)$ DOF. To compute it, the principle of virtual work says to augment \eqref{eqn:grizzle:LagrangeNoControl} with a Lagrange multiplier \begin{equation}
\label{eqn:grizzle:LagrangeNoControlWithMultiplier}
D(q) \ddot{q} + C(q,\dot{q})\dot{q} + G(q) = \left(\frac{\partial h(q)}{\partial q}\right)^T \lambda,
\end{equation}
where $\lambda$ is obtained by setting the second derivative of the constraint along solutions of the model to zero, that is,
\begin{align}
0 &= \frac{d^2h}{dt^2} \nonumber \\
\label{eqn:grizzle:SetAccelerationZero}
&= \frac{\partial h(q)}{\partial q} \ddot{q} + \frac{\partial }{\partial q}\left( \frac{\partial h(q)}{\partial q}\dot{q} \right)\dot{q}.
\end{align}
%The explicit calculation of $\lambda$ is not necessary here, but can be found in the Appendix.
Indeed, substituting the model \eqref {eqn:grizzle:LagrangeNoControlWithMultiplier} into \eqref{eqn:grizzle:SetAccelerationZero} and solving \eqref{eqn:grizzle:SetAccelerationZero} for the Lagrange multiplier yields
\begin{equation}
\label{eqn:grizzle:LagrangeMultiplier}
 \lambda^\ast =\Lambda^{-1} (q)\left[ \frac{\partial h(q)}{\partial q}\Big( C(q,\dot{q})\dot{q} + G(q) \Big) - \frac{\partial }{\partial q}\left( \frac{\partial h(q)}{\partial q}\dot{q} \right)\dot{q} \right],
\end{equation}
where
\begin{equation}
\label{eqn:grizzle:LagrangeMultiplierSecondPart}
\Lambda(q)=\left(\frac{\partial h(q)}{\partial q} D(q)^{-1} \frac{\partial h(q)}{\partial q}^T \right)
\end{equation}
is \textit{automatically invertible} from the regularity of $h$ and the positive definiteness of $D(q)$.


 The expression for the reduced-order model can be made more explicit if we assume for simplicity that
 %there exist a parametrization $\qconstrained$, $\qfree$ in which
 the holonomic constraint can be expressed as
\begin{equation}
\label{eqn:grizzle:HolonomicConstraintInq1q2}
0 = \qconstrained - h_d(\qfree),
\end{equation}
 for a choice of configuration variables $(\qconstrained,\qfree)$, with the constrained coordinates $\qconstrained \in \Q_{\rm c} \subset \mathbb{R}^k$, the free coordinates $\qfree \in \Q_{\rm f} \subset \mathbb{R}^{N-k}$, and such that a diffeomorphism $F:\Q_{\rm c} \times  \Q_{\rm f} \to \Q$ exists.
  In this case, the constraint is always regular and the constraint manifold becomes  \textbf{[It is diffeomorphic to $\Q_{\rm f}$. Worth saying?]}
\begin{equation}
\label{eqn:grizzle:ConstraintManifoldInq1q2}
\tilde{\Q}=\left\{q \in \Q~|~ q = F(h_d(\qfree),\qfree),~\qfree \in Q_{\rm f}  \right\}.
\end{equation}
Applying the configuration constraint along a trajectory of the model yields a constraint on velocity, which, using the chain rule, can be written as
\begin{align}
\label{eqn:cc:ConstraintVelocity}
\dot{q} & = \left(  \frac{\partial F(h_d(\qfree),\qfree)}{\partial \qconstrained} \frac{\partial h_d(\qfree)}{\partial \qfree}+\frac{\partial F(h_d(\qfree),\qfree)}{\partial \qfree} \right)\dqfree\\
&=: J_c(\qfree) \dqfree.
\end{align}
In addition, using the chain rule again, there is a constraint on acceleration,
\begin{align}
\label{eqn:cc:ConstraintAcceleration}
\ddot{q}&=J_c(\qfree) \ddqfree+ H_c(\qfree,\dqfree),
\end{align}
where $H_c(\qfree,\dqfree)$ contains quadratic terms in velocity resulting from the derivative.

Taking into account the constraints on configuration, velocity and acceleration, the reduced-order model on $T\tilde{\Q}$ \textbf{[ $T\Q_{\rm f}$???]}can be written as
\begin{equation}
\label{eqn:grizzle:ReducedMechanicalModel}
\tilde{D}(\qfree) \ddqfree + \tilde{H}(\qfree, \dqfree)=0,
\end{equation}
where
\begin{align}
 \tilde{D}(\qfree) &:= \left. J_c(\qfree)^T D(q) J_c(\qfree) \right|_{ q=F(h_d(\qfree),\qfree)}, \nonumber \\
 \tilde{H}(\qfree, \dqfree) &:= \left. J_c(\qfree)^T  \Big(H(q, \dot q) +  D(q) H_c(\qfree,\dqfree) \Big) \right|_{\begin{array}{l} q=F(h_d(\qfree),\qfree)\\\dot{q}=J_c(\qfree) \dqfree\end{array}}, \nonumber
 \end{align}
and
$$H(q, \dot q):=C(q,\dot q) \dot q + G(q).$$
The right-hand side of the dynamic model \eqref{eqn:grizzle:ReducedMechanicalModel} is zero because the constraints being satisfied,
$$0=h\circ F(h_d(\qfree),\qfree),$$ 
implies that
$$0=\left. \frac{\partial h(q)}{\partial q} J_c(\qfree)\right|_{q=F(h_d(\qfree),\qfree)}.$$

The solutions of the reduced-order model \eqref{eqn:grizzle:ReducedMechanicalModel} are (exact) solutions to the full-order model \eqref{eqn:grizzle:LagrangeNoControlWithMultiplier}. Indeed, if $(\qfree(t),\dqfree(t))$ is a solution of \eqref{eqn:grizzle:ReducedMechanicalModel}, then
\begin{align}
q(t)  &= F(h_d(\qfree(t)),\qfree(t)) \nonumber \\
\dot{q}(t)&= J_c(\qfree(t)) \dqfree(t) ) \nonumber
\end{align}
is a solution of \eqref{eqn:grizzle:LagrangeNoControlWithMultiplier} with the Lagrange multiplier equal to
the unique solution of \eqref{eqn:grizzle:SetAccelerationZero}.





==> sections/4-VirtualConstraintsAndFeedback.tex <==
%\textbf{[Remark: My student Brent is now designing outputs that depend on velocity (angular momentum) in a very interesting way. When he optimizes his virtual constraints for rough ground, his controller updates step length in a continuous manner. When evaluated step-to-step, it follows rather closely the capture-point method of Jerry Pratt. Brent has a single controller that can handle $\pm 8$  cm variations step to step. The work is unpublished at the present time. We hope to submit to IEEE CDC, due date around 20 March. My point is that it may be nice to hint that more general VCs are potentially useful. ][It is very interesting, but incompatible with the way I wanted to obtain the zero dynamic based simply on the equilibrium in rotation and kinetic momentum]}
%%
%%
%
%\textbf{[Remark: Second point we might talk about: ZMP, Capture Point and other methods are based on low-dimensional approximations of the dynamics. These methods have proved to be surprisingly effective. As gaits become more rapid, and higher agility is demanded, however, more and more of the dynamics must be taken into account. HZD has already been shown to be compatible with ZMP. Brent is showing that it is compatible with CP (capture point).  A potential limitation of HZD is its emphasis on periodic motions. Discuss further? ][The fact that the reduce model contains the real dynamics of the robot is a point that we have to emphasize] }
\textbf{[Better title and content: Virtual Constrains and Zero Dynamics.~~~???? We could combine Sections 4 and 5.]}\\

\textbf{[We need a general development that parallels physical constraints. Also, the introduction that follows was re-used in our Automatica paper. If you suggest a different motivation from a robotics perspective, I can try to write it.]}\\

Any attempt to describe walking, even something as simple as the
difference between human-like walking (knees bent forward) and
bird-like walking (knees bent backward), inevitably leads to a
description of the \emph{posture} or \emph{shape} of the robot
throughout a step. In other words, a description of walking involves
at least a partial specification of the path followed in the
configuration space of the biped; see
\fig{grizzle:modeling:constraint_illustration}. The following is one
possible way to express this mathematically: let
$\bq=(q_1;\cdots;q_{\numlinks-1})$ be a set of {\it body}
coordinates for the robot and let $\thetafcn$ be the angle of some
point of the robot with respect to an inertial frame, and assume
moreover that $\thetafcn$ has been chosen so that it is strictly
monotonic throughout the step. Then the path of the robot in the
configuration space can be expressed as
%
\begin{equation}
\label{eqn:grizzle:FdbkDesignApproach:virtual_constraint}
  0=\bq - h_d(\thetafcn).
\end{equation}

A natural objective is therefore: determine a feedback controller that
drives asymptotically to zero the output function
%
\begin{equation}\label{eqn:grizzle:FdbkDesignApproach:output_fcn_structure_new_coord}
  y = h({q}) := \bq-h_d(\thetafcn).
\end{equation}

\figposturecontrol

\noindent
This leads to two questions: \textbf{[Also re-used in Automatica. :)]}
\begin{enumerate}
\item \textbf{An analysis question:}
  when will a given choice of $h_d(\thetafcn)$ lead to an asymptotically
  stable periodic orbit (i.e., a stable walking motion)?
\item \textbf{A synthesis question:}
 how to make a choice of $h_d(\thetafcn)$ that will yield an
 asymptotically stable periodic orbit meeting physically motivated
 requirements such as: energy efficiency; the robot walks at a desired
 speed; and the reaction forces at the leg end are such that the
 contact between the stance and the ground behaves as a pivot?
\end{enumerate}
%
Addressing the first question leads to the notion of the hybrid zero
dynamics, the focus of this chapter. A finite parametrization of
possible paths $h_d(\theta,\parama)$ via \Bezier\ polynomials and the
use of parameter optimization have been employed to address the second
question.


==> sections/5-VirtualConstraintsAndZeroDynamics.tex <==
Physical constraints in a mechanism guide the motion along a constraint surface, but do not impose a specific evolution with respect to time. This property seems particularly well adapted to locomotion. First of all, any attempt to describe walking, even something as simple as the
difference between human-like walking (knees bent forward) and
bird-like walking (knees bent backward), inevitably leads to a
description of the \emph{posture} or \emph{shape} of the robot
throughout a step. In other words, a description of walking involves
at least a partial specification of the path followed in the
configuration space of the biped.

Secondly, in a controller based upon tracking of a time trajectory, if a disturbance were to affect the robot and
causes its motion to be retarded with respect to the planned motion, the feedback system
is then obliged to play catch up in order to regain synchrony with the reference trajectory. Presumably,
what is more important is the orbit of the robot's motion, that is, the path in state space traced out
by the robot, and not the slavish notion of time imposed by a reference trajectory (think about how
you respond to a heavy gust of wind when walking). A preferable situation, therefore, would be for
the control system in response to a disturbance to drive the motion back to the periodic orbit, but not to attempt
otherwise re-synchronizing the motion with respect to time.

With these motivations in mind, a controller based on virtual constraints is now presented. This section parallels the developments in the previous section, but this time for a model with actuation. In particular, the action of contact forces and moments is replaced by actuator torques or forces. The imposed constraints will be virtual because they exist as lines of code in an embedded controller and can be modified on the fly without any physical changes to the robot. While the constraints imposed are virtual, in the authors' opinion, they are as natural as physical constraints.

\subsection{Virtual constraints}
\label{sec:grizzle:ZD:VC}

Since the robot has $k$ independent actuators, $k$ virtual constraints can be generated by the actuators. The virtual constraints are expressed as outputs applied to the model \eqref{eqn:grizzle:modeling:model_walk}, and a feedback controller must be designed that drives asymptotically to zero the output function. In order to emphasize the parallels between virtual and physical constraints, the output is written as
%
\begin{equation}\label{eqn:grizzle:FdbkDesignApproach:output_fcn_structure_new_coord}
  y = h({q}) := \aq-h_d(\uq),
\end{equation}
where $\aq \in \Q_{\rm c} \subset \mathbb{R}^k$, and $\uq \in \Q_{\ulbl} \subset \mathbb{R}^{N-k}$ with $(\aq, \uq)$ forming  a set of generalized configuration variables for the robot (i.e., such that a diffeomorphism $F:\Q_{\rm c} \times  \Q_{\ulbl} \to \Q$ exists). The interpretation is that $\aq$ represents a collection of variables that one wishes to ``control'' or ``regulate'', while $\uq$ is a complementary set of variables that remain ``free''. Later, a special case of $h_d(\uq)$ will be introduced that highlights a \textit{gait phasing variable}, which makes it easier to interpret the virtual constraint in many instances.

The configuration constraint surface for the virtual constraints is identical to the case of physical constraints in \eqref{eqn:grizzle:ConstraintManifoldInq1q2}. Adding the velocities to the configuration variables gives the \textit{zero dynamics manifold}
\begin{align}
\label{eqn:grizzle:VC:ZeroDynManifold}
\zdmanifold:&=\{(q,\dot{q}) \in T\Q~| y = h(q) = 0, ~\dot{y}=\frac{\partial h(q)}{\partial q}\dot{q}=0\} \nonumber \\
&=\{(q,\dot{q}) \in T\Q~| q=F_c(\uq), \dot{q}=J_c(\uq) \duq, ~~(\uq, \duq) \in T\Q_{\ulbl} \},
\end{align}
which is diffeomorphic to $T\Q_{\ulbl}$. The terminology zero dynamics manifold comes from \cite{BYRNESC91}.


The torque  $u^\ast $ required to remain on the zero dynamics manifold is computed by substituting the controlled model \eqref{eqn:grizzle:modeling:mech_model_swing_phase} into \eqref{eqn:grizzle:SetAccelerationZero} and solving for the input yielding $\ddot{y}=0$. This gives
\begin{equation}
\label{eqn:grizzle:VC:eq_torque_star} u^\ast =\Big(\frac{\partial h(q)}{\partial
q}D^{-1}(q)B\Big)^{-1}\left( {  \frac{\partial }{\partial q}\left( \frac{\partial h(q)}{\partial q}\dot{q} \right)\dot{q}+\frac{\partial h(q)}{\partial
q}D^{-1}(q)H(q,\dot {q})} \right).
\end{equation}
For $u^\ast$ to be well defined, the decoupling matrix
\begin{equation}
\label{eqn:grizzle:VC:decouplingMatrix} A(q): = \frac{\partial h(q)}{\partial
q}D^{-1}(q)B
\end{equation}
must be invertible\footnote{In the control literature, the output is said to have vector relative degree two. More general constraints can be handled.}. In the case of physical constraints, the invertibility of  \eqref{eqn:grizzle:LagrangeMultiplierSecondPart} was automatic as long as the constraint was regular. With virtual constraints, \textit{the invertibility of the decoupling matrix is not automatic} and must be checked. Numerous examples exist, nevertheless, that show it is straightforward to meet this condition. Reference \cite[Chap.~6]{WGCCM07} shows how to compute the decoupling matrix without inverting the inertia matrix.

Another difference with physical constraints is that it is possible for the system to be either initialized off the virtual constraint surface or perturbed off it.  Feedback is therefore required to asymptotically drive the state of the robot to the constraint surface. The feedforward term $u^\ast$  can be modified to an input-output linearizing controller  \cite[Chap.~5]{WGCCM07},
\begin{equation}
\label{eqn:grizzle:VC:eq_torque} u=u^\ast - A(q)^{-1}\left(\frac{K_p }{\varepsilon ^2}y+\frac{K_d }{\varepsilon
}\dot {y}\right),
\end{equation}
which results in
\begin{equation}
\label{eqn:grizzle:VC:eq_closed_loop}
    \ddot {y}+\frac{K_d }{\varepsilon }\dot
{y}+\frac{K_p }{\varepsilon ^2}y=0.
\end{equation}
A richer set of feedback controllers based on control Lyapunov functions is given in \cite{ames2014rapidly}.

Like physical constraints, under certain regularity conditions, virtual constraints induce a low-dimensional invariant model of the swing-phase dynamics. The low-dimensional model is called the \textit{zero dynamics} in the nonlinear control literature \cite{BYRNESC91}. The main novelty required in biped locomotion arises from the hybrid nature of the models, which gives rise to the \textit{hybrid zero dynamics} \cite{WEGRKO03}.



The zero dynamics of the hybrid model
\eqn{grizzle:modeling:full_hybrid_model_walking} with output
\eqn{grizzle:FdbkDesignApproach:output_fcn_structure_new_coord} are
developed in a two-step process. First, the zero dynamics of the
(non-hybrid) nonlinear model consisting of the swing phase dynamics
\eqn{grizzle:modeling:model_walk} and the output
\eqn{grizzle:FdbkDesignApproach:output_fcn_structure_new_coord} are
characterized, and then, second, an impact invariance condition is
imposed on the swing-phase zero dynamics manifold in order to obtain
the hybrid zero dynamics.


\subsection{The Swing Phase Zero Dynamics}
\label{sec:grizzle:ZD:SS}
%
The objective is to characterize the swing-phase model
\eqref{eqn:grizzle:modeling:mech_model_swing_phase} restricted to the constraint surface \eqref{eqn:grizzle:VC:ZeroDynManifold}. The zero dynamics, by definition, reflects the internal dynamics when the output is identically zero, meaning the system evolves on the constraint surface. The development is analogous to the case of physical constraints, once the invertibility of a key matrix is established.


\begin{proposition} Let $B^\perp$ be a $(N-k) \times N$ matrix of rank $N-k$ such that $B^\perp B=0$ and suppose that the decoupling matrix \eqref{eqn:grizzle:VC:decouplingMatrix} is invertible at a point $q$. Then the following matrices are each $N \times N$ and have rank $N$:
$$\left[ \begin{array}{c} \frac{\partial h(q)}{\partial q}  \\ B^\perp D(q)\end{array} \right], ~
%%
\left[ \begin{array}{c} \frac{\partial h(q)}{\partial q} D^{-1}(q) \\ B^\perp \end{array} \right],~and~~
%%
\left[ \begin{array}{cc} \frac{\partial h(q)}{\partial q} D^{-1}(q) B & ~~~~\frac{\partial h(q)}{\partial q} D^{-1}(q) \left(B^\perp \right)^T\\ 0 & B^\perp  \left(B^\perp \right)^T \end{array} \right],~
%%
$$
\end{proposition}

The proof is sketched. Multiplying the leftmost matrix by the inverse of $D(q)$ gives the matrix in the middle. Multiplying the matrix in the middle by the full rank matrix $[B~|\left(B^\perp \right)^T]$ gives the rightmost matrix. This matrix is full rank because it is block upper triangular with the upper left block being the decoupling matrix, which has full rank by assumption, and the lower right block has full rank by standard properties of matrices. This completes the proof.

Multiplying the matrix on the left by the Jacobian of $F_c:  \Q_{\ulbl} \to \Q$ and restricting to the constraint surface gives
$$\left. \left[ \begin{array}{c} \frac{\partial h(q)}{\partial q} J_c(\uq) \\ B^\perp D(q) J_c(\uq)\end{array} \right] \right|_{ q=F_c(\uq)} = \left. \left[ \begin{array}{c} 0  \\ B^\perp D(q)J_c(\uq)\end{array} \right]  \right|_{ q=F_c(\uq)},
$$
where \eqref{eqn:grizzle:OrthogonalConditionOnConstraint} has been used. The proposition and the fact that $J_c(\uq)$ has rank $N-k$ give the following result.

\begin{corollary} Let $B^\perp$ be a $(N-k) \times N$ matrix of rank $N-k$ such that $B^\perp B=0$ and suppose that the decoupling matrix \eqref{eqn:grizzle:VC:decouplingMatrix} is invertible at a point $q=F_c(\uq)$. Then the matrix
\begin{equation}
\label{eqn:grizzle:VC:BperpDjacMatrix}
\left. M(\uq):=B^\perp D(q) J_c(\uq) \right|_{ q=F_c(\uq)},
\end{equation}
is invertible.
\end{corollary}


Armed with the corollary, the calculation of the reduced-order model associated with the virtual constraints is very similar to the case of physical constraints. Multiplying the controlled system \eqref{eqn:grizzle:modeling:mech_model_swing_phase} on the left by $B^\perp$ as in \cite{shiriaev2008can,shiriaev2010transverse} gives
\begin{equation}
\label{eqn:CC:dym_zeroStep1}
  B^\perp D(q) \ddot{q} + B^\perp H(q,\dot{q}) = 0.
\end{equation}
%\textbf{[Maybe relation between $B^\perp$ and $J_c$ characterizes Lagrangian or not Lagrangian system ?]}
Using \eqref{eqn:cc:ConstraintAcceleration} and restricting to $\zdmanifold$ gives
\begin{equation}\label{eqn:CC:dym_zeroStep2}
  \left.B^\perp D(q) J_c(\uq) \ddot{\uq} + B^\perp \left[  D(q) H_c(\uq,\dot{\uq}) + H(q,\dot{q}) \right]= 0 \right|_{\begin{array}{l} q=F_c(\uq)\\ \dot{q}=J_c(\uq) \dot{\uq}\end{array}},
\end{equation}
yielding a second-order model analogous to \eqref{eqn:grizzle:ReducedMechanicalModel},
\begin{equation}
\label{eqn:CC:dym_zeroStep3}
  M(\uq) \ddot{\uq} + H_{zero}(\uq,\dot{\uq}) = 0,
\end{equation}
where
$$ H_{zero}(\uq,\dot{\uq}):= \left. B^\perp \left[  D(q) H_c(\uq,\dot{\uq}) + H(q,\dot{q}) \right] \right|_{\begin{array}{l} q=F_c(\uq)\\ \dot{q}=J_c(\uq) \dot{\uq}\end{array}}.$$

From this equation, a state variable model for the zero dynamics can be obtained. Selecting $$z=\left[\begin{array}{c} z_1\\ z_2 \end{array}\right]:=\left[\begin{array}{c} \uq\\ \duq \end{array}\right]$$
gives
\begin{align}
  \dot z & =    \left[
      \begin{array}{c}
        z_2\\
        - M^{-1}(z_1) H_{zero}(z_1,z_2)
      \end{array}\right]\\
  & =: f_{zero}(z).  \label{eqn:CC:modeling:model_zero}
\end{align}


An alternative form for the zero dynamics can be obtained from the Lagrangian nature of \eqref{eqn:grizzle:modeling:mech_model_swing_phase}. Let
$$L(q,\dot{q})=\frac{1}{2} \dot{q}^T D(q) \dot{q}- V(q)$$
denote the Lagrangian of the model. Then from Lagrange's equation
$$ \frac{d}{dt} B^\perp \frac{\partial L}{\partial \dot{q} } =  B^\perp  \frac{\partial L}{\partial q },$$
because $B^\perp B u=0$. The term $B^\perp \frac{\partial L}{\partial \dot{q} }$ is a form of \textit{generalized angular momentum}. Restricting to the zero dynamics manifold gives
$$  \dusigma  = \kappa(\uq,\duq),$$
where
\begin{align} \usigma&:=M(\uq) \duq \nonumber \\
\kappa(\uq,\duq) &:= \left. B^\perp  \frac{\partial L(q,\dot{q}) }{\partial q } \right|_{
\begin{array}{l} q=F_c(\uq)\\ \dot{q}=J_c(\uq) \dot{\uq}\end{array}
}. \nonumber
\end{align}
Choosing the zero dynamics coordinates as
$$z=\left[\begin{array}{c} z_1\\ z_2 \end{array}\right]:=\left[\begin{array}{c} \uq\\ \usigma \end{array}\right]$$
gives
\begin{align}
  \dot z & =    \left[
      \begin{array}{c}
        M^{-1}(z_1) z_2\\
        \bar{\kappa}(z_1,z_2)
      \end{array}\right] \label{eqn:CC:modeling:model_zeroAlternative}\\
  & =: f_{zero}(z),   \nonumber
\end{align}
where $\bar{\kappa}(z_1,z_2) = \kappa(z_1, M^{-1}(z_1)z_2)$.



\noindent \textbf{Remark:}
An alternative expression for the torque $u^\ast$ on the zero dynamics manifold can be given. Let $B^+$ be the pseudoinverse of the full rank matrix $B$. Then
\begin{equation}
\label{eqn:grizzle:VC:ustarFromZD}
 u^\ast = \left.B^+ D(q) J_c(\uq) \ddot{\uq} + B^+ \left[H(q,\dot{q}) + D(q) H_c(\uq,\dot{\uq}) \right] \right|_{\begin{array}{l} q=F_c(\uq)\\\dot{q}=J_c(\uq) \dot{\uq}\end{array}} .
\end{equation}
In other words, the control signal required to remain on the zero dynamics manifold can be recovered directly from knowledge of the solution to any one of \eqref{eqn:CC:dym_zeroStep3}, \eqref{eqn:CC:modeling:model_zero}, or \eqref{eqn:CC:modeling:model_zeroAlternative}.

A similar methodology can be used to calculate the torque insuring the convergence toward the virtual constraints. The control law objective is:
\begin{equation}
\label{eqn:grizzle:VC:eq_closed_loop_a}
    \ddot {y}+\frac{K_d }{\varepsilon }\dot
{y}+\frac{K_p }{\varepsilon ^2}y=0.
\end{equation}

By definition of the virtual constraint, the output and its derivatives are
\begin{align}
  y &=  \aq-h_d(\uq),\\
  \dot y &= \dot \aq - \frac{\partial h_d(\uq)}{\partial \uq} \dot \uq, \\
  \ddot y &= \ddot \aq - \frac{\partial h_d(\uq)}{\partial \uq} \ddot \uq  - \frac{\partial}{\partial \uq} (\frac{\partial h_d(\uq)}{\partial \uq} \dot \uq)\dot \uq,
\end{align}

Thus using equation \eqref {eqn:grizzle:VC:eq_closed_loop_a}, one can defined the desired acceleration for the controlled variable  denoted $w$, by:

\begin{equation}
w= \frac{\partial h_d(\uq)}{\partial \uq} \ddot \uq - \frac{\partial}{\partial \uq} (\frac{\partial h_d(\uq)}{\partial \uq} \dot \uq)\dot \uq-\frac{K_d }{\varepsilon } (\dot \aq- \frac{\partial h_d(\uq)}{\partial \uq} \dot \uq) -\frac{K_p }{\varepsilon ^2}(\aq-h_d(\uq)),
\end{equation}
and the control law will be designed in order to achieve $\ddot \aq= w$.
 
In the case of virtual constraints, $w$ is composed of two parts, one corresponding to a feedforward term du to the acceleration of the free variable $\uq$ and one corresponding  to a classical feedback term. 
When calculating the torque to applied, the state of the robot is known, but not its acceleration, thus $w$ will be written as:
\begin{equation}
\label{eq:CC:w}
w= \frac{\partial h_d(\uq)}{\partial \uq} \ddot \uq + w_k(q, \dot q),
\end{equation}
to  highlight the fact that $\ddot \uq$ must be determined in a preliminary step to be able to calculate $u$. This acceleration can not be chosen but is created by the non actuated joint.
The dynamic model is known as function of the variable q, thus the diffeomorphism F defined in section \ref{sec:grizzle:PhysicalConstraints} is used to express the desired joint acceleration $w_q$ as function of $w$ and $\ddot \uq$:

\begin{equation}
w_q = \frac{\partial F(q)}{\partial \aq} w+ \frac{\partial F(q)}{\partial \uq} \ddot \uq + \frac{\partial }{\partial q} ( \frac{\partial F(q)}{\partial q} \dot q)\dot q
\end{equation}

Using equation \eqref{eq:CC:w}, we can write:
\begin{equation}
w_q  = (\frac{\partial F(q)}{\partial \aq}  \frac{\partial h_d(\uq)}{\partial \uq} + \frac{\partial F(q)}{\partial \uq} ) \ddot \uq + \frac{\partial F(q)}{\partial \aq} w_k(q, \dot q) +  \frac{\partial }{\partial q} ( \frac{\partial F(q)}{\partial q} \dot q)\dot q
\end{equation}
or
\begin{equation}
w_q =J_{cr}(q) \ddqfree+ H_{cor}(q,\dot q),
\end{equation}
It can be noted that $J_{cr}$ is calculated similarly to $J_c$ in \eqref{eqn:cc:ConstraintVelocity} but evaluated at the current configuration.

Using \eqref{eqn:CC:dym_zeroStep1}, in order to have $\ddot q= w_q$, $\ddot \uq$ must satisfy :
\begin{equation}
  B^\perp D(q) J_{cr}(q) \ddot \uq+ B^\perp D(q) H_{cor}(q,\dot q) + B^\perp H(q,\dot{q}) = 0.
\end{equation}

thus
\begin{equation}
\ddot \uq= - (  B^\perp D(q) J_{cr}(q) ) ^{-1} (B^\perp D(q) H_{cor}(q,\dot q) + B^\perp H(q,\dot{q}) )
\end{equation}

This value can be used to calculate the torque by:
\begin{equation}
 u= B^+ D(q) J_{cr}(q) \ddot \uq+ B^+ D(q) H_{cor}(q,\dot q) + B^+ H(q,\dot{q})
\end{equation}

\noindent \textbf{Remark:} The choice of the $\aq$ a $\uq$ as linear function of $q$ simplify largely the calculation of $F$ and its derivative and thus of the controlled law and of the zero dynamics.
 
\subsection{The Hybrid Zero Dynamics}
\label{sec:grizzle:ZD:Hybrid}
%

\begin{figure}[t!]
  \centering %\hspace{1.5cm}
  \subfloat[]{\includegraphics[width=.4\textwidth]{Figures_HZD/HybridInvariantZ.jpg}} \hspace{.5cm}
  \subfloat[]{\includegraphics[width=.4\textwidth]{Figures_HZD/Convergence2Z.jpg}}
  \caption{In (a) hybrid invariant manifold.  In (b), as $||y(t);\dot{y}(t)||$ tends to zero, the solution of the closed-loop system approaches the zero dynamics manifold, $\zdmanifold$.}
  \label{fig:grizzle:ZDand}
\end{figure}

To obtain the hybrid zero dynamics, the zero dynamics manifold must be
\emph{invariant under the impact map}, that is
%
\begin{equation}\label{eqn:grizzle:impact_invar_cond}
  \impactmap (\poincaresection \cap \zdmanifold) \subset \zdmanifold.
\end{equation}
%
This condition means that when a solution evolving on $\zdmanifold$ meets the switching surface, $\poincaresection$, the new initial condition arising from the impact map is once again on $\zdmanifold$.

\begin{definition}[Hybrid zero dynamics \cite{WEGRKO03}]
Consider the hybrid model \eqref{eqn:grizzle:modeling:full_hybrid_model_walking} and
output \eqref{eqn:grizzle:FdbkDesignApproach:output_fcn_structure_new_coord}.
Suppose that the decoupling matrix
\eqref{eqn:grizzle:VC:decouplingMatrix} is invertible and
let $\zdmanifold$ and $\dot z = \fzero(z)$ be the associated zero
dynamics manifold and zero dynamics of the swing phase model.  Suppose
that $\poincaresection \cap \zdmanifold$ is a smooth, co-dimension one,
embedded submanifold of $\zdmanifold$. Suppose furthermore that $\impactmap
(\poincaresection \cap \zdmanifold) \subset \zdmanifold.$ Then the
nonlinear system with impulse effects,
%
\begin{equation}\label{eqn:grizzle:zero_dynamics:reduced_hybrid_model}
  \Sigma_\zero: \begin{cases}
    \begin{aligned}
      \dot z & = \fzero(z), &    z^- & \notin \poincaresection\cap \zdmanifold\\
      z^+ & = \impactmapzero(z^-), & z^- & \in \poincaresection\cap \zdmanifold,
    \end{aligned}
    \end{cases}
\end{equation}
%
with $\impactmapzero:= \left. \impactmap \right|_{\poincaresection\cap \zdmanifold}$, is the \emph{hybrid zero
dynamics}\index{zero dynamics!hybrid}\index{hybrid zero dynamics}.
\end{definition}

The invariance condition \eqref{eqn:grizzle:impact_invar_cond} is equivalent to
\begin{align}
0=&h\circ \impactmappos(q) \\
0=& \left. \frac{\partial h(\bar{q})}{\partial q} \right|_{\bar{q}=\impactmappos(q)} \impactmapvel(q)\, \dot{q}
\end{align}
for all $(q;\dot{q})$ satisfying
\begin{align}
 h(q) =0, ~~\frac{\partial h(q)}{\partial q} \dot{q} =& 0 \\
\pswingfootv(q) = 0,~~\vswingfootv(q, \dot{q})<& 0.
\end{align}
At first glance, these conditions appear to be very hard to meet. In the case of models with one degree of underactuation (i.e., $k=N-1$), however, it is known that if a single non-trivial solution of the zero dynamics satisfies these conditions, then all solutions of the zero dynamics will satisfy them \cite[Thm.~5.2]{WGCCM07}. In the case of systems with more than one degree of underactuation, systematic methods have been developed which modify the virtual constraints ``at the boundary'' and allow the conditions to be met \cite{MOGR08}. Very straightforward implementations of the result are presented in a robotics context in \cite{CHGRSHIH09} and \cite{GrGr2015ACC}.

\noindent \textbf{Remark:} When low-dimensional pendulum models are used for gait design, they \textit{approximate} the swing phase dynamics and the impact map is ignored. The zero dynamics is an \textit{exact} low-dimensional model that captures the underactuated nature of the robot. Presumably, one could use it without insisting on the impact invariance condition \eqref{eqn:grizzle:impact_invar_cond}. To the knowledge of the authors, this has not been done.

%It is to be noted that Hybrid zero dynamics conditions are not satisfied for arbitrary choice of the virtual constraints.
%We now consider two different cases. In the case of one degree of underactuation (planar robot in sagittal plane), convenient choice of virtual constraint leads to Hybrid zero dynamics. In the case of higher degree of under actuation, a step by step modification of virtual constraint is required to produce Hybrid zero dynamics.
%
%When there is only one degree of under actuation then $(\poincaresection \cap \zdmanifold) $ reduced to a manifold of dimension 1. Since in $\zdmanifold$ the joint configuration can be parametrized by $\uq$, and in $\poincaresection$ a geometric constraint on the hight of the foot must be satisfied, there exist only a finite number of solution $\uq$ defining the configuration belonging to  $(\poincaresection \cap \zdmanifold) $.
%The virtual constraint has to be defined such that these values of $\uq$ denoted $\theta^-$ and $\theta^+$ correspond to the final and the initial configuration are such that :
%\begin{equation}
%\label{eq:CC:condpos}
%F(h_d(\theta^+),\theta^+)  = \impactmappos (F(h_d(\theta^-),\theta^-))
%\end{equation}
%To satisfy the Hybrid zero dynamics conditions, the virtual constraint must also satisfied the condition on velocity:
%\begin{equation}
%\label{eq:CC:condvit}
%J_c(\theta^+) \propto \impactmapvel (F(h_d(\theta^-),\theta^-)) J_c(\theta^-)
%\end{equation}
%where $\propto$ means is proportionel to.
%
%If this conditions \eqref{eq:CC:condpos}, \eqref{eq:CC:condpos} are satisfied, then  $\impactmap (\poincaresection \cap \zdmanifold) \subset \zdmanifold$ for any perturbation on $\uq$, $\dot \uq$. In any case, the configuration at impact will be the same, and the joint velocity will change proportionnaly and the state after impact will belong on $\zdmanifold$.
%
%When there is more degree of under actuation then $(\poincaresection \cap \zdmanifold) $ is a manifold of dimension $2 N - 2 k-1$, thus the configuration at impact is not constant and the condition for Hydrid zero dynamics cannot be meet. Condition extended from \eqref{eq:CC:condpos}, \eqref{eq:CC:condpos} can be used to insure that there exist
%one state $q_{f0}$, $\dot {q_{f0}}$ belonging to $(\poincaresection \cap \zdmanifold) $ such that after impact the state where belongs to $\zdmanifold $ but this condition can not be satisfied for any state in $(\poincaresection \cap \zdmanifold) $. Since the constraint are virtual and produced by the actuator, we propose to modify the virtual constraint from $\aq=h_d(\uq)$ to $\aq=h_d(\uq)+h_c(\uq)$. $h_c(\uq)$ is a correction of the virtual constraint that is defined at the beginning of each step, such that the state after impact belongs to the zero dynamics associated to the modified constraint \cite{CHGRSHIH09}. This modification affects the beginning of the single support phase only. It prescribes how the control law must join the initial virtual constraint, it avoids large torque that can exist in presence of tracking error and allows the zeros dynamics to perfectly predict the joint evolution.












==> sections/5-ZeroDynamics.tex <==
The zero dynamics of the hybrid model
\eqn{grizzle:modeling:full_hybrid_model_walking} with output
\eqn{grizzle:FdbkDesignApproach:output_fcn_structure_new_coord} are
developed in a two-step process. First, the zero dynamics of the
(non-hybrid) nonlinear model consisting of the swing phase dynamics
\eqn{grizzle:modeling:model_walk} and the output
\eqn{grizzle:FdbkDesignApproach:output_fcn_structure_new_coord} are
characterized, and then, second, an impact invariance condition is
imposed on the swing-phase zero dynamics manifold in order to obtain
the hybrid zero dynamics. For general hybrid systems and output
functions, this approach to forming a hybrid zero dynamics is less
general than directly applying the output zeroing definition of
Isidori et al. \cite{BYRNESC91,ISIDORIA95,ISMO88}. From results in
\cite{WEGRKO03,WESTERVELTE07b}, however, it can be deduced that for
an $N$-degree of freedom biped model with one degree of
underactuation and an $N-1$ dimensional output vector of the form
\eqn{grizzle:FdbkDesignApproach:output_fcn_structure_new_coord}, if
there exists at least one periodic solution of the hybrid model
\eqn{grizzle:modeling:full_hybrid_model_walking} that zeros the
output and is transversal to $\poincaresection$, then the approach
followed here and the definition used in \cite{ISIDORIA95} are
equivalent.


\subsection{The Swing Phase Zero Dynamics}
\label{sec:grizzle:ZD:SS}
%
The objective is to characterize the zero dynamics manifold and
associated restriction dynamics for the swing-phase model
\eqn{grizzle:modeling:model_walk} and output
\eqn{grizzle:FdbkDesignApproach:output_fcn_structure_new_coord}. The zero
dynamics, by definition, reflects the internal dynamics when the output are zeroed.

\subsection{The Hybrid Zero Dynamics}
\label{sec:grizzle:ZD:Hybrid}
%
\figManifoldsAndRabbit

To obtain the hybrid zero dynamics, the zero dynamics manifold must be
\emph{invariant under the impact map}, that is
%
\begin{equation}\label{eqn:grizzle:impact_invar_cond}
  \impactmap (\poincaresection \cap \zdmanifold) \subset \zdmanifold.
\end{equation}
%
If $\poincaresection \cap \zdmanifold$ is nonempty, then, due to the
form of the output \eqn{grizzle:FdbkDesignApproach:output_fcn_structure_new_coord},
$\poincaresection \cap \zdmanifold$ is a smooth one-dimensional
embedded submanifold of $T\tilde{\Q}$ if, and only, if
$\pswingfootv(h_d(\theta),\theta)$ has constant rank on its zero
set. Furthermore, when the decoupling matrix is invertible, the
following statements are equivalent \cite{WEGRKO03}:
%
\renewcommand{\labelenumi}{(\alph{enumi})}
\begin{enumerate}
\item \eqn{grizzle:impact_invar_cond} holds;
\item $h\circ\impactmap |_{(\poincaresection \cap \zdmanifold)} = 0$ and
 $L_fh\circ\impactmap|_{(\poincaresection \cap \zdmanifold)}=0$; and
\item there exists at least one point $(q^-_0;\dot q^-_0) \in
 \poincaresection\cap \zdmanifold$ such that $\bar{\sigma}_\numlinks
 \neq 0$, $h\circ\impactmappos(q^-_0) = 0$, and
 $L_fh\circ\impactmap(q^-_0,\dot q^-_0)=0$.
\end{enumerate}

\begin{definition}[Hybrid zero dynamics \cite{WEGRKO03}]
Consider the hybrid model \eqn{grizzle:modeling:full_hybrid_model_walking} and
output \eqn{grizzle:FdbkDesignApproach:output_fcn_structure_new_coord}.
Suppose that the decoupling matrix
\eqn{grizzle:within_stride_ctrl:decoupling_matrix_MPFL} is invertible and
let $\zdmanifold$ and $\dot z = \fzero(z)$ be the associated zero
dynamics manifold and zero dynamics of the swing phase model.  Suppose
that $\poincaresection \cap \zdmanifold$ is a smooth, one-dimensional,
embedded submanifold of $\TQ$. Suppose further that $\impactmap
(\poincaresection \cap \zdmanifold) \subset \zdmanifold.$ Then the
nonlinear system with impulse effects,
%
\begin{equation}\label{eqn:grizzle:zero_dynamics:reduced_hybrid_model}
  \Sigma_\zero: \begin{cases}
    \begin{aligned}
      \dot z & = \fzero(z), &    z^- & \notin \poincaresection\cap \zdmanifold\\
      z^+ & = \impactmap(z^-), & z^- & \in \poincaresection\cap \zdmanifold,
    \end{aligned}
    \end{cases}
\end{equation}
%
with state manifold $\zdmanifold$, is the \emph{hybrid zero
dynamics}\index{zero dynamics!hybrid}\index{hybrid zero dynamics}.
\end{definition}

\subsection{Closed-loop stability with zero dynamics}

\input{sections/StabilityProof.tex}





==> sections/6-AnalysisZeroDynamics.tex <==

This section first presents the relation between the stability of a periodic solution in the full-order model in relation to the hybrid zero dynamics. The stability of periodic orbits within the hybrid zero dynamics is subsequently analyzed.


\subsection{Closed-loop stability with zero dynamics}

\input{sections/StabilityProof.tex}


\subsection{How much of this do we need?}

In the walking, the under actuation considered comes from the contact between the leg tip and the ground that is modeled as passive. Depending on the type of contact modeled, the degree of under actuation can varies from 1 to 3.
We have one degree of actuation for planar case or rotation around a edge of the foot; two degrees of under actuation for modeling of a passive ankle \cite{}, and tree for punctual contact \cite{}.
The equilibrium in rotation of the robot around the contact point  $O$ gives the following equation:
\begin{equation}
\label{eq:dyn_sig-3D}
	\left\{
	\begin{array}{l}
\sigma_{O}=\sum_{i=1}^{n_c} \textbf{I}_{G_i}{\Omega}_i+\sum_{i=1}^{n_c}m_iV_{G_i} \times {G_i{O}} \\
{\dot{{\sigma}}_{O}}\ + m{{V}_O}\times {V}_G=\sum_{i=1}^{n_c}{O G_i} \times {m}_i g +M_O\\
	\end{array}
	\right.
\end{equation}
where $\sigma_{O}$ is the $(3 \times 1)$ vector of angular momentum around $O$ expressed in a fixed frame. $n_c$ is the number of link of the robot. For each link $i$ : $m_i$ is the mass, ${I}_{G_i}$ is the inertia tensor calculated around the mass centre denoted $G_i$, $V_{G_i}$ is the linear velocity of the mass center, ${\Omega}_i$ is the angular velocity and  ${O G_i}$ is the vector that linked $O$ and $G_i$. $G$ is the global mass center and $V_G$ its linear velocity, $m$ is the global mass. $g$ is the gravity acceleration. $M_O$ is the moment exerted by the ground, for a punctual contact this
term is null. A moment of friction can be modeled to avoid rotation around the vertical axis. if the contact point $O$ is fixed, its velocity $V_O$ is zero and the second equation can be simplified.
This model can be used to obtain the zeros dynamic equation without writing of the complete dynamic model, in a simpler form than \eqref{eqn:CC:dym_zero}.

For simplicity, we detail here, how this can be done, only the case of one degree of under actuation, corresponding to a free rotation along a fixed axis $y$. Based on the equation \eqref{eq:dyn_sig-3D}, it is possible to write:
\begin{equation}
\label{eq:dyn_sig}
	\left\{
	\begin{array}{l}
         \sigma =S(q) \dot q \\
	 \dot \sigma= - m g x(q) \\
	\end{array}
	\right.
\end{equation}
where  $\sigma$ denotes  the angular momentum around a fixed axis $y$, and $x$ is the distance between the mass center of the robot and the axis , $m$ is the mass of the robot and $S(q)$ is a ${N \times 1}$ vector defining the $ \sigma$ which is a linear quantity with respect to $\dot q$.

Using the virtual constraints \eqref{eq:dyn_sig} becomes:
\begin{equation}
\label{eq:dyn_sig_zero}
	\left\{
	\begin{array}{l}
         \sigma =S(F(h_d(\uq),\uq)) J_c(\uq) \dot{\uq} \\
	 \dot \sigma= - m g x(F(h_d(\uq),\uq)) \\
	\end{array}
	\right.
\end{equation}

From this equation, a state space form of the zeros dynamics can be expressed, with $z=\left[\begin{array}{c} \uq\\ \sigma \end{array}\right]$ :

\begin{eqnarray}
  \dot z & = &  \left[
      \begin{array}{c}
        \left(S(F(h_d(\uq),\uq)) J_c(\uq) \right)^{-1} \sigma \\
        - m g x(F(h_d(\uq),\uq))
      \end{array}\right] \\
  & =: & f_{zero}(z)  \label{eqn:CC:modeling:model_zero_2}
\end{eqnarray}

The choice of the variable $\uq$ and of the virtual constraint must be such that the matrix $\left(S(F(h_d(\uq),\uq)) J_c(\uq) \right)$ is invertible. Similar condition exist to write equation \eqref{eqn:CC:modeling:model_zero}.


\subsection{One degree of underactuation}
\label{sec:grizzle:ZD:Orbits}
%%%%%%%%%%%*******************

\textbf{[Let's try to make this shorter. ]}


\textbf{[ While 1 DUA always yields a Lagrangian zero dynamics, for 2 or more, it is rarely Lagrangian. Hence, no matter what we write down, it is not a mechanical system. This may be interesting to point out, because it is probably non-intuitive for people to think of non-mechanical ``template models'' in the sense of Koditschek and Full.]}


In this section, the case of one degree of underactuation, that appears in the study of walking in saggital plane will be developed, since this case is now, well-known and can be treated analytically to conduct to stability condition. Even if the generalization to more complex (3D) case is not strait forward, the stability condition obtained is probably also meaningful for more general case.

On $\zdmanifold$, we have seen that the zero dynamics can be written under the form \eqref{eqn:CC:modeling:model_zero_2} with a state vector  $z=\left[\begin{array}{c} \uq\\ \sigma \end{array}\right]$.

%\begin{eqnarray}
%  \dot z & = &  \left[
%      \begin{array}{c}
%        \left(S(F(h_d(\uq),\uq)) J_c(\uq) \right)^{-1} \sigma \\
%        - m g x(F(h_d(\uq),\uq))
%      \end{array}\right] \\
%  & =: & f_{zero}(z)
%\end{eqnarray}
%

It follows that the swing phase zero
dynamics is
\begin{subequations}\label{eqn:grizzle:zero_dynamics:zd_states}
 \begin{eqnarray}
   \dot \uq  & = & \zdone(\uq)\sigma \label{eqn:grizzle:zero_dynamics:zd_state_1} \\
   \dot \sigma & = & \zdtwo(\uq) \label{eqn:grizzle:zero_dynamics:zd_state_2},
 \end{eqnarray}
\end{subequations}
%
where
%
\begin{subequations}\label{eqn:grizzle:within_stride_ctrl:kappa_terms}
  \begin{eqnarray}
    \kappa_{1}(\uq) & = & \left(S(F(h_d(\uq),\uq)) J_c(\uq) \right)^{-1}\label{eqn:grizzle:within_stride_ctrl:kappa_1} \\
    \kappa_{2}(\uq) & = & - m g x(F(h_d(\uq),\uq))
  \end{eqnarray}    \label{eqn:grizzle:within_stride_ctrl:kappa_2}
 \end{subequations}
To insure the invertibility of $\left(S(F(h_d(\uq),\uq)) J_c(\uq) \right)$, $\uq$ is chosen as the absolute angle of a virtual leg connecting the hip and the point of contact denoted $\theta$, this angle is monotonic in normal walk, the actuated angle are defined by virtual constraint and the function $F$ is identity.

The single support ends when the swing leg touches the ground, this geometric condition on $\zdmanifold$ can be satisfied when $\theta=\theta^-$.
\begin{equation}
  \poincaresection \cap \zdmanifold  =
  \left\{(\uq^-;\sigma^-)~|~\uq^-=\theta^-,\sigma^- \in
    \real{}\right\}
\end{equation}

 Due to the invariance of the zero dynamics manifold under the impact map, after the relabeling the we have:
\begin{equation}
\label{grizzle:zero_dynamics:1}
\uq^+ = \theta^+
\end{equation}

and  $\theta^-$ and $\theta^+$ satisfy
%
\begin{subequations}
\begin{align}
\pswingfootv(h_d(\theta^-),\theta^-))&=0, &\pswingfooth(h_d(\theta^-),\theta^-)&>0,\\
\pswingfootv(h_d(\theta^+),\theta^+))&=0, &\pswingfooth(h_d(\theta^+),\theta^+)&<0.
\end{align}
\end{subequations}

The impact map has been defined in section \ref{sec:grizzle:model:DS} under a general form. This form can be complete by a property of conservation of angular momentum. With an impact where the swing leg touches the ground and the previous stance leg leaves the ground, the reaction force exerted by the ground is applied on the punctual contact on the front leg only. As a consequence the angular momentum around this punctual contact is conserved.
The instantaneous double support is the instant of change of support, with state variable $\sigma$, the point around which $\sigma$ is calculated changes since it is the tip of the the stance leg. As a consequence we have, for the 3D case :
\begin{equation}
\sigma_{O'}= \sigma_{O} + m {V}_G \times  {O O'}
\end{equation}
where $O$ is the contact point before impact and $O'$ after.

and for the case studied :
\begin{equation}
\sigma^+=\sigma^- + m d \dot z^-
\end{equation}
where $d$ is the distance between the following contact point along axis $x$ and $\dot z$ the vertical velocity of the mass center just before impact. Since the vertical velocity is linear with respect to joint velocity which are proportional to $\dot \uq$ or $\sigma$ we can write:

\begin{equation}
\sigma^+=\sigma^- + m d \frac{d z}{d q}J_c(\uq) \left(S(F(h_d(\uq),\uq)) J_c(\uq) \right)^{-1} \sigma^-
\end{equation}
or
\begin{equation}
\label{grizzle:zero_dynamics:2}
\sigma^+= \deltazero \sigma^-
\end{equation}

where $\deltazero<1$ when $\dot z^-<0$, or when the vertical velocity is directed downward. The motion corresponding to the linear inverted pendulum 3DLIP, largely used in control of humanoïd robot, consider only motion such that $z(t)$ is constant thus such that $\deltazero=1$. This king of motion do not lead to stable walk with the proposed approach.

%In the local coordinates $(\zdcoord_1;\zdcoord_2)$,
%$\poincaresection\cap \zdmanifold$ and
%${\impactmap:(\zdcoord_1^-;\zdcoord_2^-) \to
%(\zdcoord_1^+;\zdcoord_2^+)}$ simplify to
%%
%\begin{subequations}
%\begin{eqnarray}
%  \poincaresection \cap \zdmanifold & = &
%  \left\{(\zdcoord_1^-;\zdcoord_2^-)~|~\zdcoord_1^-=\theta^-,\zdcoord_2^- \in
%    \real{}\right\}\\
%  \zdcoord_1^+ & = & \theta^+ \label{eqn:grizzle:zero_dynamics:xi_1+}\\
%  \zdcoord_2^+ & = & \deltazero \, \zdcoord_2^-, \label{eqn:grizzle:zero_dynamics:xi_2+}
%\end{eqnarray}
%\end{subequations}
%%
%where $\deltazero$ is a constant that may be readily computed using
%\twoeqn{grizzle:modeling:delta}{grizzle:FdbkDesignApproach:output_fcn_structure_new_coord}

%
The hybrid zero dynamics is thus given by
\eqn{grizzle:zero_dynamics:zd_states} during the swing phase, and at impact
with $\poincaresection \cap \zdmanifold$, the re-initialization rules
\eqref{grizzle:zero_dynamics:1} and \eqref{grizzle:zero_dynamics:2} are applied.

For $\theta^+ \le \zdcoord_1 \le \theta^- $, define
%
\begin{equation}\label{eqn:grizzle:zero_dynamics:Vzero}
  \PEzero(\uq) :=
  -\int_{\theta^+}^{\uq}\frac{\zdtwo(\zdcoord)}{\zdone(\zdcoord)}\,
  d\zdcoord.
\end{equation}
%
A straightforward computation shows that ${\cal L}_{\rm zero} :=
\KEzero - \PEzero$ \cite{WEGRKO03}, where
%
\begin{equation}\label{eqn:grizzle:zero_dynamics:lagrangian}
  \KEzero =
  \frac{1}{2} \sigma ^2,
\end{equation}
%
is a Lagrangian\index{zero dynamics!Lagrangian} of the swing-phase
zero dynamics \eqn{grizzle:zero_dynamics:zd_states}. This implies, in
particular, that the total energy ${\cal H}_{\rm zero} := \KEzero +
\PEzero$ is constant along solutions of the swing-phase zero
dynamics. Note that the energy ${\cal H}_{\rm zero}$ is not the energy of the initial system, which is not constant since actuator torque are used to create the virtual constraints.

The analysis of periodic orbits of the hybrid zero dynamics forms the
basis for proposing feedback laws that induce exponentially stable
walking motions in the full-dimensional hybrid model. Take the
\Poincare\ section to be $\poincaresection \cap \zdmanifold$ and let
%
\begin{equation}
  \rho: \poincaresection \cap \zdmanifold \to \poincaresection \cap \zdmanifold
\end{equation}
%
denote the \Poincare\ (first return) map\footnote{This is in general a
partial map.} of the hybrid zero dynamics. Using the fact that the
total energy ${\cal H}_{\rm zero}$ is constant along solutions of the
continuous portion of the dynamics, the \Poincare\ map may be shown to
be
%
\begin{equation}\label{eqn:grizzle:zero_dynamics:poincarezdyn}
  \rho(\zeta^-) = \deltazero^2\,\zeta^- - \PEzero(\theta^-),
\end{equation}
%
where $\zeta^- := \frac{1}{2} (\sigma^-)^2$, and its domain of
definition is
%
\begin{equation}\label{eqn:grizzle:zero_dynamics:domain}
  {\cal D}_\zero= \left\{ \zeta^- > 0~\big|~\deltazero^2 \, \zeta^- - \PEzeromax > 0 \right\},
\end{equation}
%
where
%
\begin{equation}
  \PEzeromax := \max_{\theta^+ \le \uq \le \theta^-} \PEzero(\uq).
\end{equation}
%
The domain ${\cal D}_\zero$ is non-empty if, and only if,
$\deltazero^2>0$.
%
Whenever $\deltazero^2 < 1$, the fixed point of
\eqn{grizzle:zero_dynamics:poincarezdyn},
%
\begin{equation} \label{eqn:grizzle:zero_dynamics:p_nonlinear_fixed_point}
  \zeta^* := -\frac{\PEzero(\theta^-)}{1-\deltazero^2},
\end{equation}
%
will be exponentially stable as long as it belongs to ${\cal
D}_\zero$. The conditions for there to exist an exponentially stable
periodic orbit of \eqn{grizzle:zero_dynamics:reduced_hybrid_model} are thus
%
\begin{subequations}\label{eqn:grizzle:zero_dynamics:zd_conds}
  \begin{gather}\label{eqn:grizzle:zero_dynamics:zd_cond1}
    \frac{\deltazero^2}{1-\deltazero^2}\PEzero(\theta^-) + \PEzeromax < 0\\
    0 < \deltazero^2 < 1.\label{eqn:grizzle:zero_dynamics:zd_cond2}
  \end{gather}
\end{subequations}

The choice of the virtual constraints defined the sequence of configuration for the biped, one unique motions satisfying these constraints and the under-actuation exists it is defined by equation \eqref{eqn:grizzle:zero_dynamics:p_nonlinear_fixed_point}.

Periodic orbits of the hybrid zero dynamics are periodic orbits of
the full-dimensional model. Two different feedback controllers are
provided in \cite{MORRISB05,WEGRKO03} for exponentially stabilizing
these orbits in the full-dimensional model, \eqn{grizzle:modeling:model_walk}.

\subsection{Higher degrees of underactuation}

Jessy can make a few remarks, perhaps????


==> sections/6-AnalysisZeroDynamics_v02.tex <==

This section first presents the relation between the stability of a periodic solution in the full-order model in relation to the hybrid zero dynamics. The stability of periodic orbits within the hybrid zero dynamics is subsequently analyzed.


\subsection{Closed-loop stability with zero dynamics}

\input{sections/StabilityProof.tex}


%\subsection{How much of this do we need?}
%
%In the walking, the under actuation considered comes from the contact between the leg tip and the ground that is modeled as passive. Depending on the type of contact modeled, the degree of under actuation can varies from 1 to 3.
%We have one degree of actuation for planar case or rotation around a edge of the foot; two degrees of under actuation for modeling of a passive ankle \cite{}, and tree for punctual contact \cite{}.
%The equilibrium in rotation of the robot around the contact point  $O$ gives the following equation:
%\begin{equation}
%\label{eq:dyn_sig-3D}
%	\left\{
%	\begin{array}{l}
%\sigma_{O}=\sum_{i=1}^{n_c} \textbf{I}_{G_i}{\Omega}_i+\sum_{i=1}^{n_c}m_iV_{G_i} \times {G_i{O}} \\
%{\dot{{\sigma}}_{O}}\ + m{{V}_O}\times {V}_G=\sum_{i=1}^{n_c}{O G_i} \times {m}_i g +M_O\\
%	\end{array}
%	\right.
%\end{equation}
%where $\sigma_{O}$ is the $(3 \times 1)$ vector of angular momentum around $O$ expressed in a fixed frame. $n_c$ is the number of link of the robot. For each link $i$ : $m_i$ is the mass, ${I}_{G_i}$ is the inertia tensor calculated around the mass centre denoted $G_i$, $V_{G_i}$ is the linear velocity of the mass center, ${\Omega}_i$ is the angular velocity and  ${O G_i}$ is the vector that linked $O$ and $G_i$. $G$ is the global mass center and $V_G$ its linear velocity, $m$ is the global mass. $g$ is the gravity acceleration. $M_O$ is the moment exerted by the ground, for a punctual contact this
%term is null. A moment of friction can be modeled to avoid rotation around the vertical axis. if the contact point $O$ is fixed, its velocity $V_O$ is zero and the second equation can be simplified.
%This model can be used to obtain the zeros dynamic equation without writing of the complete dynamic model, in a simpler form than \eqref{eqn:CC:dym_zero}.
%
%For simplicity, we detail here, how this can be done, only the case of one degree of under actuation, corresponding to a free rotation along a fixed axis $y$. Based on the equation \eqref{eq:dyn_sig-3D}, it is possible to write:
%\begin{equation}
%\label{eq:dyn_sig}
%	\left\{
%	\begin{array}{l}
%         \sigma =S(q) \dot q \\
%	 \dot \sigma= - m g x(q) \\
%	\end{array}
%	\right.
%\end{equation}
%where  $\sigma$ denotes  the angular momentum around a fixed axis $y$, and $x$ is the distance between the mass center of the robot and the axis , $m$ is the mass of the robot and $S(q)$ is a ${N \times 1}$ vector defining the $ \sigma$ which is a linear quantity with respect to $\dot q$.
%
%Using the virtual constraints \eqref{eq:dyn_sig} becomes:
%\begin{equation}
%\label{eq:dyn_sig_zero}
%	\left\{
%	\begin{array}{l}
%         \sigma =S(F(h_d(\uq),\uq)) J_c(\uq) \dot{\uq} \\
%	 \dot \sigma= - m g x(F(h_d(\uq),\uq)) \\
%	\end{array}
%	\right.
%\end{equation}
%
%From this equation, a state space form of the zeros dynamics can be expressed, with $z=\left[\begin{array}{c} \uq\\ \sigma \end{array}\right]$ :
%
%\begin{eqnarray}
%  \dot z & = &  \left[
%      \begin{array}{c}
%        \left(S(F(h_d(\uq),\uq)) J_c(\uq) \right)^{-1} \sigma \\
%        - m g x(F(h_d(\uq),\uq))
%      \end{array}\right] \\
%  & =: & f_{zero}(z)  \label{eqn:CC:modeling:model_zero_2}
%\end{eqnarray}
%
%The choice of the variable $\uq$ and of the virtual constraint must be such that the matrix $\left(S(F(h_d(\uq),\uq)) J_c(\uq) \right)$ is invertible. Similar condition exist to write equation \eqref{eqn:CC:modeling:model_zero}.


\subsection{Special Case of One Degree of Underactuation}
\label{sec:grizzle:ZD:Orbits}
%%%%%%%%%%%*******************

When there is only one degree of underactuation, the restricted Poincar\'e map \text{$\rho :=
P^{\epsilon}|_{\poincaresection \cap \zdmanifold}$} is one-dimensional and can be computed in closed form. While one degree of underactuation is primarily a ``planar'' (2D) robot phenomenon, it has also been used in 3D robots \cite{Zutven:PHD} with both single and (nontrivial) double support phases.


The analysis here is from \cite[Chap.~6]{WGCCM07}, which shows that in the case of one-degree of underactuation, the zero dynamics can be written in a particularly simple form. Let $\theta$ be a configuration variable tied to the world frame, such as the absolute angle of the line connecting the stance hip to the end of the stance leg, and let $\sigma$ be the generalized angular momentum conjugate to $\theta$. Then in the coordinates $(\theta, \sigma)$, \eqref{eqn:CC:modeling:model_zeroAlternative} becomes
\begin{subequations}\label{eqn:grizzle:zero_dynamics:zd_states}
 \begin{eqnarray}
   \dot \theta  & = & \zdone(\theta)\sigma \label{eqn:grizzle:zero_dynamics:zd_state_1} \\
   \dot{\sigma} & = & \zdtwo(\theta) \label{eqn:grizzle:zero_dynamics:zd_state_2},
 \end{eqnarray}
\end{subequations}
%
where $\zdtwo$ is now \textit{independent of angular momentum}. Assume the virtual constraints have been selected such that the zero dynamics admit a periodic orbit, as in Theorem \ref{thm:grizzle:StabilityFromHZD}. It can be shown that $ \dot \theta $ and $\sigma$ will not change signs. Assume furthermore there exists a single point $\theta^-$ such that the swing foot height decreases to zero, with a strictly negative impact velocity in the vertical direction. In this case, \cite[Chap.~6]{WGCCM07} shows that the impact surface in the zero dynamics can be written
\begin{equation}
  \poincaresection \cap \zdmanifold  =
  \left\{(\theta^-;\sigma^-)~|~\sigma^- \in \real{}\right\}.
\end{equation}
For $(\theta^-;\sigma^-) \in \poincaresection \cap \zdmanifold$, let
$$(\theta^+;\sigma^+) = \impactmapzero(\theta^-;\sigma^-).$$

The impact map of Sect. \ref{sec:grizzle:model:DS}, which is based on \cite{HUMA94}, respects conservation of angular momentum (see \cite[Eqn.~(3.20)]{WGCCM07}). It follows that
\begin{equation}
\label{grizzle:zero_dynamics:AngularMomentumTransfer0}
\sigma^+=\sigma^- + m d \dot z^-
\end{equation}
where $d$ is the distance between the feet (measured along the $x$-axis) and $\dot{z}$ the vertical velocity of the center of mass just before impact. In general, $\dot{z}$ is linear with respect to joint velocities, and on $\zdmanifold$, it is therefore proportional to $\dot{\theta}$. Hence,  using \eqref{eqn:grizzle:zero_dynamics:zd_state_1} and the chain rule,
\begin{align}
\label{grizzle:zero_dynamics:AngularMomentumTransfer1}
\sigma^+&=\sigma^- + m d \frac{d z(\theta^-)}{d \theta} \zdone(\theta^-)\sigma^- \\
\label{grizzle:zero_dynamics:AngularMomentumTransfer2}
\sigma^+&=: \deltazero \sigma^-,
\end{align}
where it is noted that $\deltazero<1$ when $\dot z^-<0$, that is, when the vertical velocity of the center of mass is directed downward at the end of the step.


%In the local coordinates $(\zdcoord_1;\zdcoord_2)$,
%$\poincaresection\cap \zdmanifold$ and
%${\impactmap:(\zdcoord_1^-;\zdcoord_2^-) \to
%(\zdcoord_1^+;\zdcoord_2^+)}$ simplify to
%%
%\begin{subequations}
%\begin{eqnarray}
%  \poincaresection \cap \zdmanifold & = &
%  \left\{(\zdcoord_1^-;\zdcoord_2^-)~|~\zdcoord_1^-=\theta^-,\zdcoord_2^- \in
%    \real{}\right\}\\
%  \zdcoord_1^+ & = & \theta^+ \label{eqn:grizzle:zero_dynamics:xi_1+}\\
%  \zdcoord_2^+ & = & \deltazero \, \zdcoord_2^-, \label{eqn:grizzle:zero_dynamics:xi_2+}
%\end{eqnarray}
%\end{subequations}
%%
%where $\deltazero$ is a constant that may be readily computed using
%\twoeqn{grizzle:modeling:delta}{grizzle:FdbkDesignApproach:output_fcn_structure_new_coord}

%
The hybrid zero dynamics is thus given by
\eqn{grizzle:zero_dynamics:zd_states} during the swing phase, and at impact
with $\poincaresection \cap \zdmanifold$, the re-initialization rule
\eqref{grizzle:zero_dynamics:AngularMomentumTransfer2} is applied. For $\theta^+ \le \zdcoord_1 \le \theta^- $, define
%
\begin{equation}\label{eqn:grizzle:zero_dynamics:Vzero}
  \PEzero(\theta) :=
  -\int_{\theta^+}^{\uq}\frac{\zdtwo(\zdcoord)}{\zdone(\zdcoord)}\,
  d\zdcoord.
\end{equation}
%
A straightforward computation shows that ${\cal L}_{\rm zero} :=
\KEzero - \PEzero$ \cite{WEGRKO03}, where
%
\begin{equation}\label{eqn:grizzle:zero_dynamics:lagrangian}
  \KEzero =
  \frac{1}{2} \sigma ^2,
\end{equation}
%
is a Lagrangian\index{zero dynamics!Lagrangian} of the swing-phase
zero dynamics \eqn{grizzle:zero_dynamics:zd_states}. This implies, in
particular, that the total energy ${\cal E}_{\rm zero} := \KEzero +
\PEzero$ is constant along solutions of the swing-phase zero
dynamics. \emph{Note that the energy ${\cal E}_{\rm zero}$ is not the total energy of the initial system evaluated on the zero dynamics.} Indeed, the total energy of the original system is not constant along solutions because actuator power is being injected to create the virtual constraints. One might call ${\cal E}_{\rm zero} $ pseudo-energy.

The analysis of periodic orbits of the hybrid zero dynamics is based on the restricted \Poincare\ map. Take the
\Poincare\ section to be $\poincaresection \cap \zdmanifold$ and let
%
\begin{equation}
  \rho: \poincaresection \cap \zdmanifold \to \poincaresection \cap \zdmanifold
\end{equation}
%
denote the \Poincare\ (first return) map of the hybrid zero dynamics. Using the fact that the
total energy ${\cal E}_{\rm zero}$ is constant along solutions of the
swing phase zero dynamics, the \Poincare\ map is shown in \cite[pp.~129]{WGCCM07} to
be
%
\begin{equation}\label{eqn:grizzle:zero_dynamics:poincarezdyn}
  \rho(\zeta^-) = \deltazero^2\,\zeta^- - \PEzero(\theta^-),
\end{equation}
%
where $\zeta^- := \frac{1}{2} (\sigma^-)^2$, and its domain of
definition is
%
\begin{equation}\label{eqn:grizzle:zero_dynamics:domain}
  {\cal D}_\zero= \left\{ \zeta^- > 0~\big|~\deltazero^2 \, \zeta^- - \PEzeromax > 0 \right\},
\end{equation}
%
where
%
\begin{equation}
  \PEzeromax := \max_{\theta^+ \le \theta \le \theta^-} \PEzero(\theta).
\end{equation}
%
The domain ${\cal D}_\zero$ is non-empty if, and only if,
$\deltazero^2>0$.
%
Whenever $\deltazero^2 < 1$, the fixed point of
\eqn{grizzle:zero_dynamics:poincarezdyn},
%
\begin{equation} \label{eqn:grizzle:zero_dynamics:p_nonlinear_fixed_point}
  \zeta^* := -\frac{\PEzero(\theta^-)}{1-\deltazero^2},
\end{equation}
%
will be exponentially stable as long as it belongs to ${\cal
D}_\zero$. The conditions for there to exist an exponentially stable
periodic orbit of \eqn{grizzle:zero_dynamics:reduced_hybrid_model} are thus
%
\begin{subequations}\label{eqn:grizzle:zero_dynamics:zd_conds}
  \begin{gather}\label{eqn:grizzle:zero_dynamics:zd_cond1}
    \frac{\deltazero^2}{1-\deltazero^2}\PEzero(\theta^-) + \PEzeromax < 0\\
    0 < \deltazero^2 < 1.\label{eqn:grizzle:zero_dynamics:zd_cond2}
  \end{gather}
\end{subequations}
\textbf{[It seems that Fig. 6.7 from the book would be nice here.]}\\



  \begin{figure}[bt]
    \psfrag{text1}{\small $\PEzero(\theta) + \frac{1}{2}(\bar{\sigma}_\numlinks)^2$}
    \psfrag{text2}{\small $\PEzero(\theta^-) + \frac{1}{2} (\bar{\sigma}_\numlinks^*)^2$}
    \psfrag{text3}{\small $\PEzero(\theta)$}
    \psfrag{text4}{\footnotesize $\frac{1}{2}(\bar{\sigma}_\numlinks^-)^2$}
    \psfrag{text6}{\small $\underbrace{\begin{array}{c} \mbox{Impact}\\ \bar{\sigma}_\numlinks^+ = \deltazero \bar{\sigma}_\numlinks^- \end{array}}$}
    \psfrag{text5}{\footnotesize $\frac{1}{2} (\bar{\sigma}_\numlinks^+)^2$}
    \psfrag{text8}{\small $\PEzero(\theta^-)$}
    \psfrag{text9}{\small $\theta$}
    \psfrag{text10}{\small $\theta^+$}
    \psfrag{text11}{\small $\theta^-$}
    \centerline{%
    \includegraphics[scale=0.8]{Figures_HZD/energy_transfer_jwg.eps}}
    \caption%[A Qualitative Look at Stability Through Energy]
    {A qualitative look at stability through energy. The zero dynamics is Lagrangian, and thus throughout the single support phase, the corresponding total energy $\PEzero(\theta)+ \frac{1}{2} \bar{\sigma}_\numlinks^2$ is constant. At impact, the change in total energy depends on the angular momentum through $\deltazero \bar{\sigma}_\numlinks^-$ and the potential energy through $\PEzero(\theta^-)$. The total energy corresponding to the periodic orbit is  $\PEzero(\theta^-)+ \frac{1}{2} (\bar{\sigma}_\numlinks^*)^{2}$. Convergence to this total energy level occurs if the angular momentum decreases during impact, namely, $\deltazero < 1$. From the expression for the existence of a periodic orbit, $\deltazero<1 $ is equivalent to $\PEzero(\theta^-) < 0$.}
    \label{fig:within_stride_ctrl:walking_energytransfer}
  \end{figure}

\noindent \textbf{Remark:} A remarkable fact about the case of a single degree of underactuation is that \eqref{grizzle:zero_dynamics:AngularMomentumTransfer0}-\eqref{grizzle:zero_dynamics:AngularMomentumTransfer2} imply that the \emph{stability of the periodic orbit in the zero dynamics is determined by the direction of the vertical velocity of the center of mass at the end of the step, and is \emph{essentially independent} of the particular choice of virtual constraints used to realize the orbit}. Stated a bit more precisely, different  choices of $\aq$, $\uq$ and $h_d$ in \eqref{eqn:grizzle:FdbkDesignApproach:output_fcn_structure_new_coord}, each with an invertible decoupling matrix, and each defining a virtual constraint that is identically zero along the same periodic orbit, will result in a hybrid zero dynamics with the same stability properties. Other aspects of the transient behavior, such as the basin of attraction or how much control effort is required to return to the periodic orbit, may be different.

\noindent \textbf{Remark:} The motion corresponding to the 3D linear inverted pendulum (3D-LIP), widely used in control of humanoid robots, constrains the center of mass such that $z(t)$ is constant. From \eqref{grizzle:zero_dynamics:AngularMomentumTransfer1}, a similar motion in the zero dynamics would result in $\deltazero=1$, and consequently, would not be exponentially stable.

\subsection{Higher degrees of underactuation}

When two or more degrees of underactuation are considered, the dimension of the zero dynamics increases to $2(N-k)$, which is then greater than or equal to four, and the restricted Poincar\'e map \eqref{eqn:grizzle:RestrictedPoincareMap} can no longer be computed in closed form. While its numerical calculation is a valid means to analyze the stability of a periodic solution,  it is more challenging to extract information for synthesis of a stable gait.

\textbf{[Even in the case of 1 DUA, the zero dynamics is a 2-dimensional surface. The discussion on stability being idependent of the choice of constraints was made in the previous subsection.]} The second difficulty is more intrinsic to the notion of virtual constraints. One main characteristics of our control strategy is to define a path to be followed by the controlled variables rather than a motion. The temporal evolution of the biped is not a priori constrained  but defined by the respect of the role of gravity to guide the motion along the virtual constraints. As a consequence with one degree of under actuation there is a diffeomorphism between the phasing variable (time) and the variable representing the under actuation $\uq$. Assuming that a periodic cyclic motion is known, the corresponding orbit can be draw and it defines uniquely the virtual constraints, since the virtual constraint define a subspace of dimension 1. The mathematical representation, choice of variable $\uq$ and $\aq$, may differs but as long has some mathematical properties (invertibility of decoupling matrix, monotony ..) are satisfied, the resulting behavior, described on the zero dynamics, will be the same.

Recall that in the case of a single degree of underactuation, stability was determined by 

With higher degree of under actuation, the situation is more complex. For example, with two degrees of under actuation,  the control law will constraint the motion of the system to belong to a surface not a curve. Thus assuming that a periodic cyclic motion is known, the corresponding orbit can be defined but then this curve has to be included into a surface to choose the virtual constraints. Obviously there exist different way to do this, and this will affect the stability of the walk. This has been illustrated in  \cite{CHGRSHIH09}, where it has been shown that when there are two or more degrees of underactuation, stability of a periodic motion within the zero dynamics does indeed depend on the choice of the virtual constraints. The reader is referred to \cite{BURAHAGRGAGR14} for additional examples.

%In \cite{CHGRSHIH09}, it has been shown that when there are two or more degrees of underactuation, stability of a periodic motion within the zero dynamics does indeed depend on the choice of the virtual constraints. The reader is referred to \cite{BURAHAGRGAGR14} for additional examples. At the present time, for two or more two or more degrees of underactuation, the restricted \Poincare\ map must be computed in order to check stability.

Recent work in \cite{AKBUGR14} shows how to systematically search through an entire family of virtual constraints to find those that yield a stable closed-loop system. \textbf{[Add Brian's thesis.]}
Parallel to this work, choice of virtual constraint based on physical characteristics such as definition of switching condition in order to obtain a self-synchronization of motion in frontal and sagittal plane \cite{}, and regulation of the pseudo energy as it has been described in section \ref{sec:grizzle:ZD:Orbits} is also explored.

Au de la de l'étude de stabilité possibilité d'écrire une commande pour stabilisé
Modification pas à pas des contraintes
Choix de la section de Poincaré importante

Utile en particulier le steering

Pour une marche sur sol plan stabilité naturelle préférable,
pour un terrain irrégulier, amélioration possible dans le posé des pieds





==> sections/6-AnalysisZeroDynamics_v03.tex <==

This section first presents the relation between the stability of a periodic solution in the full-order model in relation to the hybrid zero dynamics. The stability of periodic orbits within the hybrid zero dynamics is subsequently analyzed.


\subsection{Closed-loop stability with zero dynamics}

\input{sections/StabilityProof.tex}


%\subsection{How much of this do we need?}
%
%In the walking, the under actuation considered comes from the contact between the leg tip and the ground that is modeled as passive. Depending on the type of contact modeled, the degree of under actuation can varies from 1 to 3.
%We have one degree of actuation for planar case or rotation around a edge of the foot; two degrees of under actuation for modeling of a passive ankle \cite{}, and tree for punctual contact \cite{}.
%The equilibrium in rotation of the robot around the contact point  $O$ gives the following equation:
%\begin{equation}
%\label{eq:dyn_sig-3D}
%	\left\{
%	\begin{array}{l}
%\sigma_{O}=\sum_{i=1}^{n_c} \textbf{I}_{G_i}{\Omega}_i+\sum_{i=1}^{n_c}m_iV_{G_i} \times {G_i{O}} \\
%{\dot{{\sigma}}_{O}}\ + m{{V}_O}\times {V}_G=\sum_{i=1}^{n_c}{O G_i} \times {m}_i g +M_O\\
%	\end{array}
%	\right.
%\end{equation}
%where $\sigma_{O}$ is the $(3 \times 1)$ vector of angular momentum around $O$ expressed in a fixed frame. $n_c$ is the number of link of the robot. For each link $i$ : $m_i$ is the mass, ${I}_{G_i}$ is the inertia tensor calculated around the mass centre denoted $G_i$, $V_{G_i}$ is the linear velocity of the mass center, ${\Omega}_i$ is the angular velocity and  ${O G_i}$ is the vector that linked $O$ and $G_i$. $G$ is the global mass center and $V_G$ its linear velocity, $m$ is the global mass. $g$ is the gravity acceleration. $M_O$ is the moment exerted by the ground, for a punctual contact this
%term is null. A moment of friction can be modeled to avoid rotation around the vertical axis. if the contact point $O$ is fixed, its velocity $V_O$ is zero and the second equation can be simplified.
%This model can be used to obtain the zeros dynamic equation without writing of the complete dynamic model, in a simpler form than \eqref{eqn:CC:dym_zero}.
%
%For simplicity, we detail here, how this can be done, only the case of one degree of under actuation, corresponding to a free rotation along a fixed axis $y$. Based on the equation \eqref{eq:dyn_sig-3D}, it is possible to write:
%\begin{equation}
%\label{eq:dyn_sig}
%	\left\{
%	\begin{array}{l}
%         \sigma =S(q) \dot q \\
%	 \dot \sigma= - m g x(q) \\
%	\end{array}
%	\right.
%\end{equation}
%where  $\sigma$ denotes  the angular momentum around a fixed axis $y$, and $x$ is the distance between the mass center of the robot and the axis , $m$ is the mass of the robot and $S(q)$ is a ${N \times 1}$ vector defining the $ \sigma$ which is a linear quantity with respect to $\dot q$.
%
%Using the virtual constraints \eqref{eq:dyn_sig} becomes:
%\begin{equation}
%\label{eq:dyn_sig_zero}
%	\left\{
%	\begin{array}{l}
%         \sigma =S(F(h_d(\uq),\uq)) J_c(\uq) \dot{\uq} \\
%	 \dot \sigma= - m g x(F(h_d(\uq),\uq)) \\
%	\end{array}
%	\right.
%\end{equation}
%
%From this equation, a state space form of the zeros dynamics can be expressed, with $z=\left[\begin{array}{c} \uq\\ \sigma \end{array}\right]$ :
%
%\begin{eqnarray}
%  \dot z & = &  \left[
%      \begin{array}{c}
%        \left(S(F(h_d(\uq),\uq)) J_c(\uq) \right)^{-1} \sigma \\
%        - m g x(F(h_d(\uq),\uq))
%      \end{array}\right] \\
%  & =: & f_{zero}(z)  \label{eqn:CC:modeling:model_zero_2}
%\end{eqnarray}
%
%The choice of the variable $\uq$ and of the virtual constraint must be such that the matrix $\left(S(F(h_d(\uq),\uq)) J_c(\uq) \right)$ is invertible. Similar condition exist to write equation \eqref{eqn:CC:modeling:model_zero}.


\subsection{Special Case of One Degree of Underactuation}
\label{sec:grizzle:ZD:Orbits}
%%%%%%%%%%%*******************

When there is only one degree of underactuation, the restricted Poincar\'e map \text{$\rho :=
P^{\epsilon}|_{\poincaresection \cap \zdmanifold}$} is one-dimensional and can be computed in closed form. While one degree of underactuation is primarily a ``planar'' (2D) robot phenomenon, it has also been used in 3D robots \cite{Zutven:PHD} with both single and (nontrivial) double support phases.


The analysis here is from \cite[Chap.~6]{WGCCM07}, which shows that in the case of one-degree of underactuation, the zero dynamics can be written in a particularly simple form. Let $\theta$ be a configuration variable tied to the world frame, such as the absolute angle of the line connecting the stance hip to the end of the stance leg, and let $\sigma$ be the generalized angular momentum conjugate to $\theta$. Then in the coordinates $(\theta, \sigma)$, \eqref{eqn:CC:modeling:model_zeroAlternative} becomes
\begin{subequations}\label{eqn:grizzle:zero_dynamics:zd_states}
 \begin{eqnarray}
   \dot \theta  & = & \zdone(\theta)\sigma \label{eqn:grizzle:zero_dynamics:zd_state_1} \\
   \dot{\sigma} & = & \zdtwo(\theta) \label{eqn:grizzle:zero_dynamics:zd_state_2},
 \end{eqnarray}
\end{subequations}
%
where $\zdtwo$ is now \textit{independent of angular momentum}. Assume the virtual constraints have been selected such that the zero dynamics admit a periodic orbit, as in Theorem \ref{thm:grizzle:StabilityFromHZD}. It can be shown that $ \dot \theta $ and $\sigma$ will not change signs. Assume furthermore there exists a single point $\theta^-$ such that the swing foot height decreases to zero, with a strictly negative impact velocity in the vertical direction. In this case, \cite[Chap.~6]{WGCCM07} shows that the impact surface in the zero dynamics can be written
\begin{equation}
  \poincaresection \cap \zdmanifold  =
  \left\{(\theta^-;\sigma^-)~|~\sigma^- \in \real{}\right\}.
\end{equation}
For $(\theta^-;\sigma^-) \in \poincaresection \cap \zdmanifold$, let
$$(\theta^+;\sigma^+) = \impactmapzero(\theta^-;\sigma^-).$$

The impact map of Sect. \ref{sec:grizzle:model:DS}, which is based on \cite{HUMA94}, respects conservation of angular momentum (see \cite[Eqn.~(3.20)]{WGCCM07}). It follows that
\begin{equation}
\label{grizzle:zero_dynamics:AngularMomentumTransfer0}
\sigma^+=\sigma^- + m d \dot z^-
\end{equation}
where $d$ is the distance between the feet (measured along the $x$-axis) and $\dot{z}$ the vertical velocity of the center of mass just before impact. In general, $\dot{z}$ is linear with respect to joint velocities, and on $\zdmanifold$, it is therefore proportional to $\dot{\theta}$. Hence,  using \eqref{eqn:grizzle:zero_dynamics:zd_state_1} and the chain rule,
\begin{align}
\label{grizzle:zero_dynamics:AngularMomentumTransfer1}
\sigma^+&=\sigma^- + m d \frac{d z(\theta^-)}{d \theta} \zdone(\theta^-)\sigma^- \\
\label{grizzle:zero_dynamics:AngularMomentumTransfer2}
\sigma^+&=: \deltazero \sigma^-,
\end{align}
where it is noted that $\deltazero<1$ when $\dot z^-<0$, that is, when the vertical velocity of the center of mass is directed downward at the end of the step.


%In the local coordinates $(\zdcoord_1;\zdcoord_2)$,
%$\poincaresection\cap \zdmanifold$ and
%${\impactmap:(\zdcoord_1^-;\zdcoord_2^-) \to
%(\zdcoord_1^+;\zdcoord_2^+)}$ simplify to
%%
%\begin{subequations}
%\begin{eqnarray}
%  \poincaresection \cap \zdmanifold & = &
%  \left\{(\zdcoord_1^-;\zdcoord_2^-)~|~\zdcoord_1^-=\theta^-,\zdcoord_2^- \in
%    \real{}\right\}\\
%  \zdcoord_1^+ & = & \theta^+ \label{eqn:grizzle:zero_dynamics:xi_1+}\\
%  \zdcoord_2^+ & = & \deltazero \, \zdcoord_2^-, \label{eqn:grizzle:zero_dynamics:xi_2+}
%\end{eqnarray}
%\end{subequations}
%%
%where $\deltazero$ is a constant that may be readily computed using
%\twoeqn{grizzle:modeling:delta}{grizzle:FdbkDesignApproach:output_fcn_structure_new_coord}

%
The hybrid zero dynamics is thus given by
\eqn{grizzle:zero_dynamics:zd_states} during the swing phase, and at impact
with $\poincaresection \cap \zdmanifold$, the re-initialization rule
\eqref{grizzle:zero_dynamics:AngularMomentumTransfer2} is applied. For $\theta^+ \le \zdcoord_1 \le \theta^- $, define
%
\begin{equation}\label{eqn:grizzle:zero_dynamics:Vzero}
  \PEzero(\theta) :=
  -\int_{\theta^+}^{\uq}\frac{\zdtwo(\zdcoord)}{\zdone(\zdcoord)}\,
  d\zdcoord.
\end{equation}
%
A straightforward computation shows that ${\cal L}_{\rm zero} :=
\KEzero - \PEzero$ \cite{WEGRKO03}, where
%
\begin{equation}\label{eqn:grizzle:zero_dynamics:lagrangian}
  \KEzero =
  \frac{1}{2} \sigma ^2,
\end{equation}
%
is a Lagrangian\index{zero dynamics!Lagrangian} of the swing-phase
zero dynamics \eqn{grizzle:zero_dynamics:zd_states}. This implies, in
particular, that the total energy ${\cal E}_{\rm zero} := \KEzero +
\PEzero$ is constant along solutions of the swing-phase zero
dynamics. \emph{Note that the energy ${\cal E}_{\rm zero}$ is not the total energy of the initial system evaluated on the zero dynamics.} Indeed, the total energy of the original system is not constant along solutions because actuator power is being injected to create the virtual constraints. One might call ${\cal E}_{\rm zero} $ pseudo-energy.

The analysis of periodic orbits of the hybrid zero dynamics is based on the restricted \Poincare\ map. Take the
\Poincare\ section to be $\poincaresection \cap \zdmanifold$ and let
%
\begin{equation}
  \rho: \poincaresection \cap \zdmanifold \to \poincaresection \cap \zdmanifold
\end{equation}
%
denote the \Poincare\ (first return) map of the hybrid zero dynamics. Using the fact that the
total energy ${\cal E}_{\rm zero}$ is constant along solutions of the
swing phase zero dynamics, the \Poincare\ map is shown in \cite[pp.~129]{WGCCM07} to
be
%
\begin{equation}\label{eqn:grizzle:zero_dynamics:poincarezdyn}
  \rho(\zeta^-) = \deltazero^2\,\zeta^- - \PEzero(\theta^-),
\end{equation}
%
where $\zeta^- := \frac{1}{2} (\sigma^-)^2$, and its domain of
definition is
%
\begin{equation}\label{eqn:grizzle:zero_dynamics:domain}
  {\cal D}_\zero= \left\{ \zeta^- > 0~\big|~\deltazero^2 \, \zeta^- - \PEzeromax > 0 \right\},
\end{equation}
%
where
%
\begin{equation}
  \PEzeromax := \max_{\theta^+ \le \theta \le \theta^-} \PEzero(\theta).
\end{equation}
%
The domain ${\cal D}_\zero$ is non-empty if, and only if,
$\deltazero^2>0$.
%
Whenever $\deltazero^2 < 1$, the fixed point of
\eqn{grizzle:zero_dynamics:poincarezdyn},
%
\begin{equation} \label{eqn:grizzle:zero_dynamics:p_nonlinear_fixed_point}
  \zeta^* := -\frac{\PEzero(\theta^-)}{1-\deltazero^2},
\end{equation}
%
will be exponentially stable as long as it belongs to ${\cal
D}_\zero$. The conditions for there to exist an exponentially stable
periodic orbit of \eqn{grizzle:zero_dynamics:reduced_hybrid_model} are thus
%
\begin{subequations}\label{eqn:grizzle:zero_dynamics:zd_conds}
  \begin{gather}\label{eqn:grizzle:zero_dynamics:zd_cond1}
    \frac{\deltazero^2}{1-\deltazero^2}\PEzero(\theta^-) + \PEzeromax < 0\\
    0 < \deltazero^2 < 1.\label{eqn:grizzle:zero_dynamics:zd_cond2}
  \end{gather}
\end{subequations}


  \begin{figure}[bt]
    \psfrag{text1}{\small $\PEzero(\theta) + \frac{1}{2}(\bar{\sigma}_\numlinks)^2$}
    \psfrag{text2}{\small $\PEzero(\theta^-) + \frac{1}{2} (\bar{\sigma}_\numlinks^*)^2$}
    \psfrag{text3}{\small $\PEzero(\theta)$}
    \psfrag{text4}{\footnotesize $\frac{1}{2}(\bar{\sigma}_\numlinks^-)^2$}
    \psfrag{text6}{\small $\underbrace{\begin{array}{c} \mbox{Impact}\\ \bar{\sigma}_\numlinks^+ = \deltazero \bar{\sigma}_\numlinks^- \end{array}}$}
    \psfrag{text5}{\footnotesize $\frac{1}{2} (\bar{\sigma}_\numlinks^+)^2$}
    \psfrag{text8}{\small $\PEzero(\theta^-)$}
    \psfrag{text9}{\small $\theta$}
    \psfrag{text10}{\small $\theta^+$}
    \psfrag{text11}{\small $\theta^-$}
    \centerline{%
    \includegraphics[scale=0.8]{Figures_HZD/energy_transfer_jwg.eps}}
    \caption%[A Qualitative Look at Stability Through Energy]
    {A qualitative look at stability through energy. The zero dynamics is Lagrangian, and thus throughout the single support phase, the corresponding total energy $\PEzero(\theta)+ \frac{1}{2} \bar{\sigma}_\numlinks^2$ is constant. At impact, the change in total energy depends on the angular momentum through $\deltazero \bar{\sigma}_\numlinks^-$ and the potential energy through $\PEzero(\theta^-)$. The total energy corresponding to the periodic orbit is  $\PEzero(\theta^-)+ \frac{1}{2} (\bar{\sigma}_\numlinks^*)^{2}$. Convergence to this total energy level occurs if the angular momentum decreases during impact, namely, $\deltazero < 1$. From the expression for the existence of a periodic orbit, $\deltazero<1 $ is equivalent to $\PEzero(\theta^-) < 0$.}
    \label{fig:within_stride_ctrl:walking_energytransfer}
  \end{figure}

\noindent \textbf{Remark:} A remarkable fact about the case of a single degree of underactuation is that \eqref{grizzle:zero_dynamics:AngularMomentumTransfer0}-\eqref{grizzle:zero_dynamics:AngularMomentumTransfer2} imply that the \emph{stability of the periodic orbit in the zero dynamics is determined by the direction of the vertical velocity of the center of mass at the end of the step, and is \emph{essentially independent} of the particular choice of virtual constraints used to realize the orbit}. Stated a bit more precisely, different  choices of $\aq$, $\uq$ and $h_d$ in \eqref{eqn:grizzle:FdbkDesignApproach:output_fcn_structure_new_coord}, each with an invertible decoupling matrix, and each defining a virtual constraint that is identically zero along the same periodic orbit, will result in a hybrid zero dynamics with the same stability properties. Other aspects of the transient behavior, such as the basin of attraction or how much control effort is required to return to the periodic orbit, may be different.

\noindent \textbf{Remark:} The motion corresponding to the 3D linear inverted pendulum (3D-LIP), widely used in control of humanoid robots, constrains the center of mass such that $z(t)$ is constant. From \eqref{grizzle:zero_dynamics:AngularMomentumTransfer1}, a similar motion in the zero dynamics would result in $\deltazero=1$, and consequently, would not be exponentially stable.

\subsection{Higher degrees of underactuation}

When two or more degrees of underactuation are considered, the dimension of the zero dynamics is then greater than or equal to four, and the restricted Poincar\'e map \eqref{eqn:grizzle:RestrictedPoincareMap} can no longer be computed in closed form. While its numerical calculation remains a valid means to analyze the stability of a periodic solution,  it is more challenging to extract information for synthesis of a gait. In addition, when there are two or more degrees of underactuation, it has been shown that stability of a periodic motion within the zero dynamics does indeed depend on the choice of the virtual constraints, in contrast to the case of one degree of underactuation analyzed above. Reference \cite{CHGRSHIH09} gives two choices of virtual constraints that result in the \textit{same periodic solution of the robot}, and yet the periodic orbit is asymptotically stable for one of the choices and unstable for the other; see \cite{BURAHAGRGAGR14} for additional examples. In each of the cited examples, stability was recovered by judiciously modifying a virtual constraint in the ``frontal plane''.

In a certain sense, the fact that stability depends on the choice of virtual constraints is the more natural situation. The surprise was really that for one degree of underactuation, the periodic orbit itself determines closed-loop stability when designing controllers on the basis of virtual constraints. Recent work in \cite{AKBUGR14} shows how to systematically search through a family of virtual constraints to find stabilizing solutions, with no restrictions of the degree of underactuation. In parallel to this work, the selection of virtual constraints and switching conditions in order to obtain ``self-synchronization'' of frontal and sagittal plane motions of an underactuated 3D biped is explored in \cite{Hamed}, along with regulation of the ``pseudo energy'' \eqref{eqn:grizzle:zero_dynamics:lagrangian}.

An alternative method to stabilize a periodic motion, adjust the rate of convergence, or improve robustness to perturbations is to modify the virtual constraints step to step. To do this, one introduces parameters $\beta$ into the virtual constraints
\begin{equation}\label{eqn:grizzle:EventBasedVCs}
  y = h({q},\beta) 
\end{equation}
in such a way that they alter step length, step width, or torso lean angle, for example \cite{WGCCM07,CHGRSHIH09}. The \Poincare\ map then depends on the parameters $\beta$, resulting in a discrete-time control system evolving on the \Poincare\ section
\begin{equation}\label{eqn:grizzle:EventBasedPoincare}
  x_{k+1}=P(x_k,\beta_k).
\end{equation}
If $x^*=P(x^*,\beta^*)$ is a fixed point, then an \textit{event-based control action} of the form
\begin{equation}\label{eqn:grizzle:EventBasedPoincareControl}
  \beta_k = \beta^* + K(x_k - x^*)
\end{equation}
can be designed on the basis of a Jacobian linearization of \eqref{eqn:grizzle:EventBasedPoincare}. The design can be done with the restricted \Poincare\ map. The same analysis and design can be carried out with the restricted \Poincare\ map \cite[pp.~107]{WGCCM07}, which is perhaps philosophically more satisfying as it is based on the low dimensional pendulum-like dynamics of the underactuated portion of the model.

\textbf{[On garde ceci.]} Cette approche appelée "Event based control " est un outil puissant mais il présente quelques limites :
Retard face a une perturbations
Difficulté d'avoir une mesure fiable.
Les modification des contraintes virtuelles sont autorisées seulement hors de la section de Poincaré, la choix de cette section influent donc sur les propriétés de cette commande.



\textbf{[Ici, On s'eloigne de l'analyse de la stabilite. Ceci parle de design, non? Pour moi cela explique pourquoi en 1 degree de sous actionnement, on n'a pas d'effet du choix des sorties alors que avec plusieurs on a un effet. On compense 1 degré par la liberté sur l'évolution temporelle mais pas plus.]} The second difficulty is more intrinsic to the notion of virtual constraints. One main characteristics of our control strategy is to define a path to be followed by the controlled variables rather than a motion. The temporal evolution of the biped is not a priori constrained  but defined by the respect of the role of gravity to guide the motion along the virtual constraints. As a consequence with one degree of under actuation there is a diffeomorphism between the phasing variable (time) and the variable representing the under actuation $\uq$. Assuming that a periodic cyclic motion is known, the corresponding orbit can be draw and it defines uniquely the virtual constraints, since the virtual constraint define a subspace of dimension 1. The mathematical representation, choice of variable $\uq$ and $\aq$, may differs but as long has some mathematical properties (invertibility of decoupling matrix, monotony ..) are satisfied, the resulting behavior, described on the zero dynamics, will be the same.

Recall that in the case of a single degree of underactuation, stability was determined by

With higher degree of under actuation, the situation is more complex. For example, with two degrees of under actuation,  the control law will constraint the motion of the system to belong to a surface not a curve. Thus assuming that a periodic cyclic motion is known, the corresponding orbit can be defined but then this curve has to be included into a surface to choose the virtual constraints. Obviously there exist different way to do this, and this will affect the stability of the walk. This has been illustrated in  \cite{CHGRSHIH09}, where it has been shown that when there are two or more degrees of underactuation, stability of a periodic motion within the zero dynamics does indeed depend on the choice of the virtual constraints. The reader is referred to \cite{BURAHAGRGAGR14} for additional examples.

%

Si on fait un parallèle entre la commande de bipède et la marche humaine, la commande HZD peut être perçue comme une commande bas niveau qui est acquise lors de l'apprentissage de la marche, et l'event based control peut être comme une supervision qui agit pour s'adapter à l'environnement. Autant il semble légitime d'utiliser cet outil pour se diriger à partir d'information intermittente  par exemple visuelle pour orienter la direction du déplacement comme dans \cite{ChingLong} ou dans des terrain très perturbés. Autant pour une marche en ligne droite dans un terrain faiblement perturbé, il semble plus pertinent de choisir les contraintes virtuelles pour avoir une marche stable sans supervision.

Remarque: le fait qu'une stabilisation soit possible via l'Event based control et la détermination de la matrice de gain k peut être une piste de modification des contraintes virtuelles pour accroître la stabilité.






==> sections/9-AdditionalMaterial.tex <==

Here are some topics where we can write 3 or 4 sentences each, with references to the literature on HZD.


\begin{enumerate}
\item Multiple phases

\item Non-trivial double support

\item Fully actuated robots

\item Two step approach to stability

\item Composition of motions

\item Uneven ground

\item Series elastic actuators

\end{enumerate}

==> sections/StabilityProof.tex <==

Consider a Lipschitz continuous feedback law
\begin{equation}
\label{eqn:grizzle:paramFeedback}
u = \alpha(x,\epsilon)
\end{equation}
that depends on a tuning parameter $\epsilon>0$ and apply it to the model \eqref{eqn:grizzle:modeling:full_hybrid_model_walking}. Let $P^\epsilon : S\to S$ be the Poincar\'e (return) map\footnote{It is in general a partial map and depends on the tuning parameter through the feedback \eqref{eqn:grizzle:paramFeedback}. It is defined by starting with a point in $S$, applying the impact map, using this as an initial condition of the closed-loop ODE, and following the flow until it first crosses $S$ at time $T_I$; see \cite[Chap.~4]{WGCCM07} for a careful definition.} of the closed-loop system, defined in the usual way. For a given $\epsilon>0$, $x^*\in S$ is a fixed point if $P^\epsilon(x^*)=x^*$, which is well-known to be equivalent to the existence of a periodic solution of the closed-loop system.

The feedback \eqref{eqn:grizzle:paramFeedback} is \textit{compatible with the zero dynamics} if
\begin{equation}
\label{eqn:grizzle:allowedFeedback}
\left. \alpha(x,\epsilon)\right|_{Z} = \left. u^\ast(x)\right|_{Z}.
\end{equation}
In this case, if $\Delta(x^*)\in Z$, then the periodic solution is independent of the tuning parameter $\epsilon$.
Based on \cite{ames2014rapidly}, the feedback is said to \textit{drive the virtual constraints rapidly exponentially to zero} if there exist constants $\beta>0$ and $\gamma>0$ such that, for each $\epsilon>0$, there exists $\delta>0$, such for all $x_0\in B_{\delta}(\Delta(x^*))$,
\begin{equation}
\label{eqn:grizzle:ExpRapidly}
||y(t,x_0), \dot{y}(t,x_0)|| \le \frac{\beta}{\epsilon} e^{-\frac{\gamma}{\epsilon }t} ||y(0),\dot{y}(0)||.
\end{equation}




\begin{theorem}(\cite{MOGR08}, \cite{ames2014rapidly}) \textbf{Determining Closed-loop Stability from the HZD}) \label{thm:grizzle:StabilityFromHZD}
Suppose that the virtual constraints \eqref{eqn:grizzle:FdbkDesignApproach:output_fcn_structure_new_coord} satisfy
\begin{enumerate}
%\setlength{\itemsep}{.05in}
\renewcommand{\labelenumi}{(\alph{enumi})}
%
\item the decoupling matrix is invertible,
\item the associated zero dynamics manifold $Z$ is hybrid invariant, and
\item there exists a point $x^*\in S\cap Z$ giving rise to a periodic orbit.
\end{enumerate}
Assume moreover that the feedback \eqref{eqn:grizzle:paramFeedback}
\begin{enumerate}
%\setlength{\itemsep}{.05in}
\renewcommand{\labelenumi}{(\alph{enumi})}
\item[(d)] is compatible with the zero dynamics in the sense of \eqref{eqn:grizzle:allowedFeedback} and
\item[(e)]  drives the virtual constraints rapidly exponentially to zero.
\end{enumerate}
Then there exists $\bar{\epsilon} > 0$ such
that for $0 < \epsilon < \bar{\epsilon}$, the following are equivalent:
\begin{enumerate}
  \renewcommand{\labelenumi}{\roman{enumi})}
      \item the periodic orbit is locally exponentially stable;
  \item $x^*$ is an exponentially stable fixed point of
  $P^{\epsilon};$ and
    \item $x^*$ is an exponentially stable fixed point of $\rho$,
\end{enumerate}
%
where the restricted Poincar\'e map
\begin{equation}
\label{eqn:grizzle:RestrictedPoincareMap}
\rho :=
P^{\epsilon}|_{\poincaresection \cap \zdmanifold}
\end{equation}
is the Poincar\'e map of the hybrid zero dynamics, is independent of the feedback, and hence is also independent of $\epsilon$.
{\vspace{-0.05in} \begin{flushright} $\Box$ \end{flushright}}
\end{theorem}


\noindent \textbf{Remark:} It is re-emphasized that periodic orbits of the hybrid zero dynamics are periodic orbits of
the full-dimensional model. Two feedback controllers are
provided in \cite{MORRISB05,WEGRKO03} for exponentially stabilizing
these orbits in the full-dimensional model, \eqref{eqn:grizzle:modeling:model_walk}, and a third family of feedback controllers is presented in \cite{ames2014rapidly}.

